Collaborative Trustworthiness for Good Decision Making in Autonomous Systems

Autonomous systems are becoming an integral part of many application domains, like in the mobility sector. However, ensuring their safe and correct behaviour in dynamic and complex environments remains a significant challenge, where systems should autonomously make decisions e.g., about manoeuvring. We propose in this paper a general collaborative approach for increasing the level of trustworthiness in the environment of operation and improve reliability and good decision making in autonomous system. In the presence of conflicting information, aggregation becomes a major issue for trustworthy decision making based on collaborative data sharing. Unlike classical approaches in the literature that rely on consensus or majority as aggregation rule, we exploit the fact that autonomous systems have different quality attributes like perception quality. We use this criteria to determine which autonomous systems are trustworthy and borrow concepts from social epistemology to define aggregation and propagation rules, used for automated decision making. We use Binary Decision Diagrams (BDDs) as formal models for beliefs aggregation and propagation, and formulate reduction rules to reduce the size of the BDDs and allow efficient computation structures for collaborative automated reasoning.

==> tex-figures/col_reliability.tex <==
\begin{figure}[]
  \centering

\begin{tikzpicture}
\begin{axis}[%
view={0}{90},
%width=\pdfw,
%height=\pdfh,
%width=8cm,
%height=7cm,
width=7cm,
height=6cm,
scale only axis,
xmin=1, xmax=8,
xlabel={Rules},
xtick=data,
xticklabels={Most-Expert, 2-Expert, 3-Expert, 4-Expert, Majority, Gravity-Point},label style={font=\small},
xticklabel style={yshift=0ex, rotate=90},
x label style={anchor=north},
ymin=0, ymax=1.3,
ylabel={Collaborative Reliability $R_i^c$}, label style={font=\small},
ymajorgrids,
legend style={at={(0.97,0.03)},anchor=south east,nodes=right}]
\addplot[only marks,mark=square*,color=blue] plot coordinates{ (2,1.037) (3,1.089) (4,1.101) (5,1.094) (6,1.12) (7,1.1015)};

\addlegendentry{Dist.1};

\addplot[only marks,mark=diamond*,color=yellow] plot coordinates{ (2,1.16853) (3,1.067) (4,1.1973) (5,1.0746) (6,1.1408) (7,1.1286)};

\addlegendentry{Dist.2};

\addplot[only marks,mark=triangle*,color=green] plot coordinates{ (2,0.6) (3,0.5) (4,0.62) (5,0.672) (6,0.63) (7,0.738)};

\addlegendentry{Dist.3};

\addplot[only marks,mark=square*,color=red] plot coordinates{ (2,0.54) (3,0.52) (4,0.692) (5,0.668) (6,0.557) (7,0.614) };

\addlegendentry{Dist.4};

\addplot [
color=black,
solid,
line width=1.0pt,
forget plot
]
coordinates{
 (1,1)(8,1) 
};
\end{axis}
\end{tikzpicture}%
\caption{Average Collaborative Reliability for Different Groups and Different Rules. For each generated group, the rules were applied, belief propagation occurred, and the results were shown. For each rule and each group, depending on the group's error distribution, the average collaborative reliability is calculated, and the lower the average collaborative reliability ratio, the better.}
\label{fig:col_reliability}
\end{figure}

==> tex-figures/diff_groups_dist.tex <==





\pgfplotsset{compat=1.18}

\begin{figure}[]
\begin{tikzpicture}
\begin{axis}[
xmajorgrids= true,
xlabel={Error Distributions},
ylabel={Distribution Groups},
xmin=0, xmax=100,
xtick={0,10,20,30,40,50,60,70,80,90,100},
yticklabels={0,20,40,60,80,100},
ymin=0, ymax=5,
ytick={1,2,3,4},
yticklabels={Dist.1, Dist.2, Dist.3, Dist.4},
]
\addplot[draw=none] gnuplot[raw gnuplot] {
plot 0; %included to avoid warning of empty plot
set table "kdensity1.dat";
plot "data1.dat" using 1:2 smooth kdensity bandwidth 1.;
unset table;
set table "kdensity2.dat";
plot "data2.dat" using 1:2 smooth kdensity bandwidth 1.;
unset table;
set table "kdensity3.dat";
plot "data3.dat" using 1:2 smooth kdensity bandwidth 1.;
unset table;
set table "kdensity4.dat";
plot "data4.dat" using 1:2 smooth kdensity bandwidth 1.;
unset table;
};

\addplot[draw=none, name path=p1, y filter/.expression={1+0.1*y}] table {kdensity1.dat};
\addplot[draw=none, name path=m1, y filter/.expression={1-0.1*y}] table {kdensity1.dat};
\addplot[blue!100] fill between [of=p1 and m1];

\addplot[draw=none, name path=p2, y filter/.expression={2+0.05*y}] table {kdensity2.dat};
\addplot[draw=none, name path=m2, y filter/.expression={2-0.05*y}] table {kdensity2.dat};
\addplot[black!10!orange!100] fill between [of=p2 and m2];

\addplot[draw=none, name path=p3, y filter/.expression={3+0.05*y}] table {kdensity3.dat};
\addplot[draw=none, name path=m3, y filter/.expression={3-0.05*y}] table {kdensity3.dat};
\addplot[black!20!green!100] fill between [of=p3 and m3];

\addplot[draw=none, name path=p4, y filter/.expression={4+0.05*y}] table {kdensity4.dat};
\addplot[draw=none, name path=m4, y filter/.expression={4-0.05*y}] table {kdensity4.dat};
\addplot[black!10!red!100] fill between [of=p4 and m4];

\end{axis}
\end{tikzpicture}
\caption{Different Groups and their Error Probability Distributions. Each group was generated independently by changing the quality of features of the agents in the group, different error distributions were obtained, as the lower the quality of features, the higher the error probability for each agent. \hl{@Omar: i dont like this figure, can you please improve it? also colors}}
\label{fig:diff_groups_dist}
\end{figure}

==> tex-figures/sum_errors_aft_coll_high_quality.tex <==
% \begin{multicols}{2}
% \begin{Figure}
% \begin{tikzpicture}
%     \begin{axis}
%     [ybar=0.3cm,
%     bar width=0.18cm,
%     width=7cm,
%     height=6cm,
%     ymin=0,
%     ymax=85,
%     yticklabel style={font=\scriptsize},
%     xtick=data,
%     xticklabels={1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17,18,19,20},
%     xticklabel style={yshift=0ex, font=\scriptsize},
%     x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
%     ylabel={Sum of Errors Performed by Experts},
%     xlabel={Experts},
%     major x tick style={opacity=0},
%     minor x tick num=1,
%     minor tick length=1 ex,
%     ymajorgrids= true,
%     legend style={
%     at={(0.50,1.02)},
%     anchor=south,
%     column sep=0ex,
%     legend columns=-1,
%     }
% ]
% \addplot [style={blue, fill=blue}] coordinates {
%     (1,40) 
%     (2,42) 
%     (3,45) 
%     (4,50)
%     (5,52)
%     (6,55)
%     (7,58)
%     (8,60)
%     (9,58)
%     (10,61)
%     (11,63)
%     (12,65)
%     (13,68)
%     (14,70)
%     (15,58)
%     (16,72)
%     (17,76)
%     (18,73)
%     (19,75)
%     (20,77)
% };
% \end{axis}
% \end{tikzpicture}
%     \centering
%     \captionsetup{width=0.9\textwidth}
%     \captionof{figure}{ \hl{@Omar: you can group both Fig 8 and Fig 9 as one Figure with a) and b) and only one caption}Sum of Individual errors performed by Experts after belief propagation over 100 iterations by a low-quality features group. The low-quality features group results in a higher sum of errors than the high-quality features group see Fig.\ref{fig:sum_errors_aft_coll_high_quality}  \hl{@Omar: in the yaxis is it the sum of errors by experts or by all group?}} 
%     \label{fig:sum_errors_aft_coll_low_quality}
% \end{Figure}
% \columnbreak
% \begin{Figure}
% \begin{tikzpicture}
%     \begin{axis}
%     [ybar=0.3cm,
%     bar width=0.18cm,
%     width=7cm,
%     height=6cm,
%     ymin=0,
%     ymax=85,
%     yticklabel style={font=\scriptsize},
%     xtick=data,
%     xticklabels={1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17,18,19,20},
%     xticklabel style={yshift=0ex, font=\scriptsize},
%     x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
%     ylabel={Sum of Errors Performed by Experts},
%     xlabel={Experts},
%     major x tick style={opacity=0},
%     minor x tick num=1,
%     minor tick length=1 ex,
%     ymajorgrids= true,
%     legend style={
%     at={(0.50,1.02)},
%     anchor=south,
%     column sep=0ex,
%     legend columns=-1,
%     }
% ]
% \addplot [style={blue, fill=blue}] coordinates {
%     (1,4) 
%     (2,5) 
%     (3,13) 
%     (4,17)
%     (5,14)
%     (6,25)
%     (7,20)
%     (8,28)
%     (9,35)
%     (10,39)
%     (11,39)
%     (12,41)
%     (13,38)
%     (14,49)
%     (15,54)
%     (16,54)
%     (17,63)
%     (18,65)
%     (19,75)
%     (20,67)
% };
% \end{axis}
% \end{tikzpicture}
% \centering
% \captionsetup{width=0.9\textwidth}
% \captionof{figure}{ \hl{@Omar: maybe here in the x-axis you talk about the ranking of experts rather than just experts}Sum of Individual errors performed by Experts after belief propagation over 100 iterations by a high-quality features group. The high-quality features group results in a lower sum of errors than the low-quality features group see Fig.\ref{fig:sum_errors_aft_coll_low_quality}}
% \label{fig:sum_errors_aft_coll_high_quality}
% \end{Figure}
% \end{multicols}


\begin{figure}[]
    \centering
    \begin{multicols}{2}
    \begin{subfigure}{0.45\textwidth}
    % \hspace{-20pt}
    \begin{tikzpicture}
    \begin{axis}
    [ybar=0.4cm,
    bar width=0.2cm,
    width=7.5cm,
    height=6cm,
    ymin=0,
    ymax=85,
    yticklabel style={font=\scriptsize},
    xtick=data,
    xticklabels={$s_{1}$, $s_{2}$,$s_{3}$,$s_{4}$,$s_{5}$,$s_{6}$,$s_{7}$,$s_{8}$,$s_{9}$,~~~$s_{10}$,~~~$s_{11}$,~~~$s_{12}$,~~~$s_{13}$,~~~$s_{14}$,~~~$s_{15}$,~~~$s_{16}$,~~~$s_{17}$,~~~$s_{18}$,~~~$~~~s_{19}$,~~~$~~~s_{20}$},
    xticklabel style={yshift=0ex, font=\tiny},
    x label style={at={(axis description cs:0.5,-0.1)},anchor=north, font=\scriptsize},
    ylabel={Sum of Errors Performed by Each Autonomous System},
    y label style={font=\scriptsize},
    xlabel={Autonomous Systems from More expert ($s_1$) to Less expert ($s_{20}$)},
    % major x tick style={opacity=0},
    % minor x tick num=1,
    % minor tick length=1 ex,
    ymajorgrids= true,
]
\addplot [style={blue, fill=blue}] coordinates {
    (1,40) 
    (2,42) 
    (3,45) 
    (4,50)
    (5,52)
    (6,55)
    (7,58)
    (8,60)
    (9,58)
    (10,61)
    (11,63)
    (12,65)
    (13,68)
    (14,70)
    (15,58)
    (16,72)
    (17,76)
    (18,73)
    (19,75)
    (20,77)
};
\end{axis}
    \end{tikzpicture}
    \centering
    % \vspace{-6pt}
    % \captionsetup{width=0.9\textwidth}
    % \captionof{figure}{ \hl{@Omar: you can group both Fig 8 and Fig 9 as one Figure with a) and b) and only one caption}Sum of Individual errors performed by Experts after belief propagation over 100 iterations by a low-quality features group (a) and by a high-quality features group (b). The low-quality features group results in a higher sum of errors than the high-quality features group see Fig.\ref{fig:sum_errors_aft_coll_high_quality}  \hl{@Omar: in the yaxis is it the sum of errors by experts or by all group?}}
    \caption{} 
    \label{fig:sum_errors_aft_coll_low_quality}
    \end{subfigure}%
    
    \columnbreak

    \begin{subfigure}{0.45\textwidth}
    % \hspace{-28pt}
    \vspace{15pt}
    \begin{tikzpicture}
    \begin{axis}
    [ybar=0.4cm,
    bar width=0.2cm,
    width=7.5cm,
    height=6cm,
    ymin=0,
    ymax=85,
    yticklabel style={font=\scriptsize},
    xtick=data,
  %  xticklabels={$s__1$, {$s__2$},$s__3$,$s__4$,$s__5$,$s__6$,$s__7$,$s__8$,$s__9$,$s__1__0$,$s__1__1$,$s__1__2$,$s__1__3$,$s__1__4$,$s__1__5$,$s__1__6$,$s__1__7$,$s__1__8$,$s__1__9$,$s__2__0$},
     xticklabels={$s_{1}$, $s_{2}$,$s_{3}$,$s_{4}$,$s_{5}$,$s_{6}$,$s_{7}$,$s_{8}$,$s_{9}$,~~~$s_{10}$,~~~$s_{11}$,~~~$s_{12}$,~~~$s_{13}$,~~~$s_{14}$,~~~$s_{15}$,~~~$s_{16}$,~~~$s_{17}$,~~~$s_{18}$,~~~$~~~s_{19}$,~~~$~~~s_{20}$},
    xticklabel style={yshift=0ex, font=\tiny},
    x label style={at={(axis description cs:0.5,-0.1)},anchor=north, font=\scriptsize},
    % ylabel={Sum of Errors Performed by Experts},
    y label style={font=\scriptsize},
    xlabel={Autonomous Systems from More expert ($s_1$) to Less expert ($s_{20}$)},
    % major x tick style={opacity=0},
    % minor x tick num=1,
    % minor tick length=1 ex,
    ymajorgrids= true,
]
\addplot [style={blue, fill=blue}] coordinates {
    (1,4) 
    (2,5) 
    (3,13) 
    (4,17)
    (5,14)
    (6,25)
    (7,20)
    (8,28)
    (9,35)
    (10,39)
    (11,39)
    (12,41)
    (13,38)
    (14,49)
    (15,54)
    (16,54)
    (17,63)
    (18,65)
    (19,75)
    (20,67)
};
\end{axis}
    \end{tikzpicture}
\centering
\captionsetup{width=0.9\textwidth}
% \vspace{-18pt}
\caption{} 
\label{fig:sum_errors_aft_coll_high_quality}
% \captionof{figure}{b}
\end{subfigure}%
    \end{multicols}
    % \vspace{-20pt}
    
\caption{Sum of Individual errors performed by each autonomous system after belief aggregation and propagation over 100 configurations by a low-quality attribute group Fig. ~\ref{fig:sum_errors_aft_coll_low_quality} \hl{@omar: here also fix numbering, the notation 18a is not nice, btw are you sure its is the sum of errors or percentage??? It should be the rror distribution}and by a high-quality attribute group Fig. ~\ref{fig:sum_errors_aft_coll_low_quality}. The low-quality attribute group results in a higher sum of errors than the high-quality attribute group.  }
\label{fig:sum_errors}
    
\end{figure}

==> tex/abstract.tex <==
%\hl{The paper should have one ping, ONE CLEAR, ONE SHARP Idea} --> so \textbf{ONE Paper = ONE Idea}

%\begin{itemize}
%        \item usually you write it last, coz it will probably change as the focus of your paper changes
 %       \item 4 sentences: state the problem, say why it is an interesting problem, say what your solution achieves, say what follows from your solution. 
  % \end{itemize}


%\hl{todo: rewrite...} \
\pagestyle{fancy}
\fancyhf{}
\fancyhead[LO,RE]{}
\hl{Zn: I don't like the "Good" in the title. It is too vague. What is good? Why not optimal? ;-) I'd rather go with performant or safe or both (trade-off).}

\hl{todo: say in the abstract that that we refer to good as safe and also performant. }
Collaboration in autonomous systems is critical to increase performance while ensuring safety. However, due to heterogeneity of their features in, e.g., perception qualities, \hl{Zn: or also their state, e.g., proximity to region of interest} some autonomous systems \hl{Zn: agents? What do you consider a system? The collection of all agents? Even if also the agents are systems, the used terminology should be clear.} have to be considered more trustworthy than others when contributing to collaboratively build  a common environmental model, especially under uncertainty. In this paper, we introduce  the idea of increasing the reliability of autonomous systems by relying on collective intelligence. We borrow concepts from social epistemology to exploit individual characteristics of autonomous systems, and define and formalize \st{at} design rules for collective \hl{Zn: or collaborative? (this term is used in title of first chapter} reasoning to achieve collaboratively increased safety, trustworthiness and good decision making.


that serves reasoning about safety at operational time, using collaboratively shared information between autonomous systems. The approach exploits the fact that autonomous systems have different quality attributes that can be used in the aggregation. 

==> tex/contrib_bdds.tex <==
\section{Peer Disagreement, Beliefs Aggregation and Propagation}

\hl{here we deal mainly with aggregation function and model of computation}

However, one of the main issues in the epistemic sense is to deal with \emph{peer disagreement}. That is, should an individual (or a system) adjusts an own belief based on additional knowledge, which can as well be contradictory, provided by other peers? In the following, we discuss how similar principles can be applied to autonomous systems.
\hl{todo: emphasize the problem of peer disagreement}

\subsection{Peer Disagreement and Beliefs Aggregation}
As mentioned previously, every autonomous system $i$ has an own belief $x_i(p)$ on a given proposition $p$. It receives as well beliefs $y_j(p)$ from other autonomous systems $j \in G_i$ belonging to a group of interest $G_i$ that we will define more precisely in the following. 

%\begin{definition} [Peer Disagreement]
\paragraph{Peer Disagreement}
Peer disagreement occurs whenever two autonomous systems $(i,j)$ have different beliefs about the same proposition $p$, that is \hl{Maybe here define peer disagreement with a condition of having at least 3 autonomous systems in the environment}
$$\exists(i,j) ~~\mbox{s.t.,} ~~x(i) \neq y (j)$$
%\end{definition}



\begin{definition} [Aggregation Rules]
The aggregation function can be defined in multiple ways. The goal of the aggregation function is to reduce peer disagreement, by adopting the beliefs of other autonomous systems when they disagree with own belief. Several aggregation rules can be defined, we use in the following the following simple aggregation function, 

%$$\odot = x_i(p) \land \neg y_1(p), ..., \neg y_k(p) \longrightarrow \neg x_i(p) $$

%$$
%\sigma(s,i) = \left\{
%    \begin{array}{ll}
%        \tau_{si} & \mbox{si } \{s,i\} \in E \\
%        \infty & \mbox{sinon.}
%    \end{array}
%\right.
%$$

$$
y_i(p) = \odot (x_i(p), ~~\forall j\in G_i~y_i^j (p) )= \left\{
    \begin{array}{ll}
        \neg x_i(p) & \mbox{if } x_i(p) \land \neg y_i^1(p)\land ...\land \neg y_i^k(p) \\
         x_i(p) & \mbox{otherwise.}
    \end{array}
\right.
$$

According to this rule, an autonomous system $i$ changes its own belief on a proposition $p$,  $x_i(p)$ when this latter disagrees with all input beliefs $y_j(p)$ belonging to the group of interest for $i$, $G_i$. 

Note that by changing own belief, \hl{this is the arithmetic equal, i am not sure if we should not write it in the boolan sense.}
$$y_i(p) = y_i^1(p)\land ...\land \neg y_i^k(p)$$
\end{definition}




\begin{definition}[Rules for Group Selection]
In order to illustrate the concept of rules, we consider in the following very simple and straightforward set of rules for belief propagation that can be applied, and discuss that, when applied, these latter do not necessarily lead to a collectively increased reliability.

\begin{itemize}
    \item "Most Expert" rule
In the most expert rule, the belief (e.g., an object has been detected) of the most "expert" autonomous system is propagated to the rest of the group, see Fig.~\ref{fig:rules}-(a). Each member of the group systematically adopts the belief of the most expert autonomous system, even if contradicting with own belief (e.g., an object has not been detected) or beliefs from other autonomous systems. The rule builds on trusting the opinion of the most expert, %(which is the most trustworthy in the group based on the quality of its feature)
as it constitutes the autonomous system which has the best quality of features in the group and which thereby considers its belief as the most trustworthy. This rule considers that only the most expert is responsible of forming a correct belief. However, one weakness of the rule is that it relies on \emph{one} single opinion and is therefore not resilient to the case where the most expert autonomous system makes an error of judgement. 

$$ \forall~~ s_i, G_i = \{s_{sup}\}$$ \hl{i think if we consider that the higher is the better .. todo check that..}

\item "n-expert" rule, 
it is $n$ of those who have better features, \hl{todo: give an example of 2-expert rule.}
$$ \forall~~ s_i, G_i = \{s_1, s_2, ... s_n\} \text{so that } s_1 > s_i, s_2 > s_i \text{ and } s_n > s_i
$$

\item "Majority" rule
In the majority rule, beliefs from all autonomous system are propagated to the rest of the group. Each autonomous systems therefore collects all beliefs including own belief and adopts the belief of the majority of the group similar to a voting mechanism, see Fig.,~\ref{fig:rules}-(b). In this case, all autonomous systems in the group are responsible of forming a correct belief. While this approach offers a given notion of fairness as all beliefs are considered, this can as well constitute the main weakness of the approach. Indeed, the majority rule considers all beliefs in the group including beliefs from less experts autonomous systems with a low quality of features. In this case all autonomous systems, including less trustworthy ones contribute to forming a correct belief. In the smart intersection example considered previously, even vehicles with a larger distance from the pedestrian or with a bad perception angle will contribute to the overall decision making process, thereby possible leading to an error in the propagated belief and overall decrease in reliability when using the majority rule for collective reasoning. 

\hl{here mention that the group of interest for every autonomous system  is the entire set }
$$ \forall~~ s_i, G_i = \mathcal{S}$$ 

\end{itemize}
 
\end{definition}

\subsection{Structuring Beliefs and Beliefs Propagation}


\begin{definition}[Belief Propagation]
    Belief propagation can be defined by applying recursively the belief aggregation function $\odot$ as defined in~\ref{def:belief-aggregation} throughout the binary decision tree. 
    \begin{equation}
        \left\{
            \begin{array}{ll}
             y_j(p) = x_j(p)    \qquad \forall j \in G_{k} 
             \\   
            y_n(p) = \odot (x_n(p), ~ y_{n-1}(p), ~y_{n-2}(p), ..., ~ y_{n-k}(p) )   \qquad \forall n \geq k \\        
            \end{array}
        \right.
    \end{equation}
\end{definition}



\begin{definition}[Rules for Group Selection]
In order to illustrate the concept of rules, we consider in the following very simple and straightforward set of rules for belief propagation that can be applied, and discuss that, when applied, these latter do not necessarily lead to a collectively increased reliability.

\begin{itemize}
    \item "Most Expert" rule
In the most expert rule, the belief (e.g., an object has been detected) of the most "expert" autonomous system is propagated to the rest of the group, see Fig.~\ref{fig:rules}-(a). Each member of the group systematically adopts the belief of the most expert autonomous system, even if contradicting with own belief (e.g., an object has not been detected) or beliefs from other autonomous systems. The rule builds on trusting the opinion of the most expert, %(which is the most trustworthy in the group based on the quality of its feature)
as it constitutes the autonomous system which has the best quality of features in the group and which thereby considers its belief as the most trustworthy. This rule considers that only the most expert is responsible of forming a correct belief. However, one weakness of the rule is that it relies on \emph{one} single opinion and is therefore not resilient to the case where the most expert autonomous system makes an error of judgement. 

$$ \forall~~ s_i, G_i = \{s_{sup}\}$$ \hl{i think if we consider that the higher is the better .. todo check that..}

\item "n-expert" rule, 
it is $n$ of those who have better features, \hl{todo: give an example of 2-expert rule.}
$$ \forall~~ s_i, G_i = \{s_1, s_2, ... s_n\} \text{so that } s_1 > s_i, s_2 > s_i \text{ and } s_n > s_i
$$

\item "Majority" rule
In the majority rule, beliefs from all autonomous system are propagated to the rest of the group. Each autonomous systems therefore collects all beliefs including own belief and adopts the belief of the majority of the group similar to a voting mechanism, see Fig.,~\ref{fig:rules}-(b). In this case, all autonomous systems in the group are responsible of forming a correct belief. While this approach offers a given notion of fairness as all beliefs are considered, this can as well constitute the main weakness of the approach. Indeed, the majority rule considers all beliefs in the group including beliefs from less experts autonomous systems with a low quality of features. In this case all autonomous systems, including less trustworthy ones contribute to forming a correct belief. In the smart intersection example considered previously, even vehicles with a larger distance from the pedestrian or with a bad perception angle will contribute to the overall decision making process, thereby possible leading to an error in the propagated belief and overall decrease in reliability when using the majority rule for collective reasoning. 

\hl{here mention that the group of interest for every autonomous system  is the entire set }
$$ \forall~~ s_i, G_i = \mathcal{S}$$ 

\end{itemize}
 
\end{definition}

\hl{-->}
We models beliefs as boolean variables. Therefore, for every autonomous system, a boolean variable represent a belief on a given proposition, e.g., “an object has been detected”. We further use Binary Decision Diagrams (BDDs) to model all possible beliefs from all autonomous systems referring to a given proposition. Fig~\ref{fig:bdd_example} depicts an example with 3 autonomous systems. Every vertex is a boolean variable representing the belief of one autonomous system, every vertex has two arcs, either the belief is assigned 1 (true) or assigned 0 (false). Each terminal vertex is labelled 0 or 1 which corresponds to the belief of the \emph{last} autonomous system. 

\hl{>--}


\begin{figure}
	\centering
  \includegraphics[scale = 0.45]
{figures/BDDs_example}
	\caption{Binary Decision Diagram (BDD) considering 3 autonomous systems.  Decision variables for autonomous system are ranked from the most expert to the least expert one. }
	\label{fig:bdd_example}
\end{figure}


Given a proposition $p$\footnote{Note that we consider so far and for the sake of simplicity, one BDD per proposition $p$}, every autonomous system $i$ believes that $p$ is true or not, that is $x_i(p)$ or not $\neg~ x_i(p)$. The set of all possible beliefs for a group of autonomous agents can be structured and modeled using Binary Decision Diagrams (BDDs)~\cite{bdds-seminal}. 


\begin{definition}[Beliefs as BDDs]
Beliefs about a given proposition are modeled as directed acyclic graphs with labeled nodes and edges as follows, 
\begin{itemize}
    \item there are two types of nodes: decision nodes and terminal nodes. 
    \item every decision node is labeled $x_i(p)$ and has two outgoing edges, one edge is labeled by 0 for \emph{false} and another is labeled 1 for {true}.
    \item a terminal node is labeled by either 0 or 1 and has no outgoing edge. A terminal node is called a 0-terminal or a 1-terminal node according to its label. 
\end{itemize}
\end{definition}

\paragraph{Ordering of Beliefs}
We consider a given order of variables in the BDDs, where for each node   $x_i(p)$ < $x_j(p)$. The order we consider should follow an order in the lattice, that is
\hl{todo: say that all variables in the BDD should satisfy this condition}
$$s_i> s_j \implies x_i(p) < x_j(p) $$
In this case, beliefs in the binary decision digram can propagate from the most expert to the least expert autonomous system according to the established lattice order. 
Terminal nodes then contain the beliefs of the \emph{last} node. 

\begin{definition}[Order of variables and group of interest]
%\hl{to define this in a recursive way we need to assume that the part of the group to which belongs the group of interest is following the experts and therefore the orders, }
We define for an autonomous system $i$, the group of interest as the set of beliefs of $k$ autonomous systems whose quality of features is better than $i$, that is $$s_i \leq \{s_{i-1}, s_{i-2}, ..., s_{i-k}\}$$
%$$G_i = \{y_{n-1}(p),~ y_{n-2}(p), ~..., ~y_{n-k}(p)\}$$ 
The set of corresponding beliefs from the defined group of interest can therefore be described as follows, 
%$$G_i = \{y_{i}^{i-1}(p),~ y_{i}^{i-2}(p), ~..., ~y_{i}^{i-k}(p) \}$$ 

$$G_i = \{y_{i-1}(p),~ y_{i-2}(p), ~..., ~y_{i-k}(p) \}$$ 


%These latter will contribute to building the beliefs 
%$$y_i (p)$,
\end{definition}




%\begin{definition}[Belief Propagation]
\paragraph{Belief Propagation}
Belief propagation can be defined by applying recursively the belief aggregation function $\odot$ as defined in~\ref{def:belief-aggregation} throughout the binary decision tree. 
%\end{definition}

\begin{equation}
\left\{
    \begin{array}{ll}
     y_j(p) = x_j(p)    \qquad \forall j \in G_{k} 
     \\   
    y_n(p) = \odot (x_n(p), ~ y_{n-1}(p), ~y_{n-2}(p), ..., ~ y_{n-k}(p) )   \qquad \forall n \geq k \\        
    \end{array}
\right.
\end{equation}


%\hl{belief propagation is about applying the aggregation rule recursively on the set of variables of the beliefs of autonomous systems. The goal is also to minimize peer disagreement through propagation}


%\hl{Belief propagation is a recursive function..}
%\hl{-----Selma: i sopped here, i am fixing notation using the bot symbol as well}
%$$
%\odot (x_i(p), \forall j\in G_i,~y_i^j (p) )= 
%\left\{
%    \begin{array}{ll}
%       % y_1(p) = x_1(p) \\
%       y_1(p) =  \odot (x_1(p), ~\bot, ..., \bot)} = x_1(p) \\
%        y_2(p) = x_2(p) \\
%        ... \\
%         y_k(p) = x_k(p) \\
%         ~  \\
%        % y_n(p) = \odot (x_n(p), \forall j\in G_i,~y_i^j (p) )
        
% y_n(p) = \odot (x_n(p), ~ y_{n-1}(p), ~y_{n-2}(p), ..., ~ y_{n-k}(p) )
         
%       % \neg x_i(p) & \mbox{if } x_i(p) \land \neg y_i^1(p)\land ...\land \neg y_i^k(p) \\
%       %  x_i(p) & \mbox{otherwise.}
%    \end{array}
%\right.
%$$

\hl{-->}
Every autonomous system receives beliefs from other autonomous systems belonging to a group of interest that can be defined based on different rules or procedures. When for example the majority rule is used, the group of interest correspond to all autonomous systems.  When an expert-based rule is used, then the group of interest refers to a (sub)set of experts. A more detailed definition will be presented in Sec.~\ref{sec:moc_model}. Every autonomous system can change its own belief after applying an aggregate function. The goal of the aggregate function is to reduce peer disagreements where an autonomous system can change its own belief to adopt the belief of the rest of the group of interest, i.e., for instance the opinion of more experts nodes. Fig~\ref{fig:aggregate_function} depicts an example of such aggregate function under peer disagreement. In this case the autonomous system $i$ changes its belief when this latter disagrees with all beliefs from other autonomous systems belonging to the group of interest. 

By reducing peer disagreement and adopting the beliefs of other autonomous systems when they contradict with own belief, we aim at reducing errors (e.g., from one autonomous system perception system) by relying on beliefs from other members of the group. The goal is to therefore increase reliability collaboratively. Note that by adopting the belief of other members of the group, an autonomous system is generally resilient to errors except for the case when multiple members of the group of interest are making errors simultaneously. A more detailed discussion regarding the choice of the group of interest, the aggregation rule and reliability will be presented in Sec.~\ref{sec:moc_model}.



\begin{figure}
	\centering
  \includegraphics[scale = 0.45]
{figures/aggregation}
	\caption{Example of an aggregate function for belief aggregation. The function considers $k$ input beliefs $y_j(p)$ on a proposition $p$.  Belief of a node $x_i(p)$ is changed if there is a disagreement with all input beliefs.}
	\label{fig:aggregate_function}
\end{figure}
\hl{>--}

\subsubsection{Belief Propagation and Transformation Rules}

\hl{-->}
The adopted order of variables in the BDDs structure follows a total order from the lattice. In this case, belief propagation in the BDDs starts from the most expert to the least expert node (or autonomous system). The aggregation function is then used by every node in the BDD to decide whether the autonomous system changes its own belief to adopt the belief of the most expert one(s). The aggregated belief is further propagated and contributes to later beliefs aggregation. 

Belief aggregation and propagation lead to a transformation of the BDD to a simpler form as depicted in Fig.~\ref{fig: ....}, where less experts adopt the belief of the most expert one (s). In that case terminal vertices correspond to the belief of the last autonomous system(s). which allows to reduce as well the complexity of systems. 


\hl{at the end of this section say that the following sections will present a detailed model and formalization of this and that the experimental section will evaluate x and y.}

\begin{figure}
	\centering
  \includegraphics[scale = 0.45]
{figures/BDDs_Reduction}
	\caption{(a): non reduced BDDs, (b): reduced BDD considering the most expert rule, (c) reduced BDD considering the 2-experts rule.}
	\label{fig: ...}
\end{figure}

\hl{>--}

We define transformation rules over the defined BDD graphs to reflect belief aggregation and propagation and which will lead to a transformation and reduction of the BDD graphs. 

\begin{enumerate}
    \item Remove duplicate terminals: eliminate all but one terminal vertex with a given label and redirect all arcs into the eliminated vertices to the remaining one ~\cite{bdd-seminal}, this rule follows the standard BDD reduction rules ~in~\cite{bdd-seminal}

    \item Every node $x_i(p)$ is replaced by $y_i(p)$ after beliefs aggregation

    \item the aggregated belief $y_i(p)$ is further propagated and contributes to beliefs aggregations.    
\end{enumerate}


\hl{maybe at the end this is a mapping from one graph to another...}

\paragraph{Belief Reduction and Convergence of Beliefs}
Aggregation and propagation rules leads to reduction of the binary tree where \emph{less experts adopt the belief of most expert one(s)}. 

%\hl{i am not sure whether this should be a lemma or a theorem. }
%\begin{Theorem}[Belief Convergence]
According to the rule defined in~\ref{...}. If we have a sequence of $k$ similar beliefs, that is $[\bar{n} -k,\bar{n}]$ so that $y_{\bar{n}-k} = ... = y_{\bar{n}}$, then all beliefs $n \geq \bar{n}$ will converge (i.e., convergence here means also that peer disagreement  will disappear after the propagation), that is 
$$\forall n \geq \bar{n}, y_{n}  = y_{\bar{n}} = $$


%\begin{proof}
We prove that by induction as follows, 
if we assume it is true at step $n$, this means that $y_{n-1}(p)= y_{n-2}(p)=... = y_{n-k}(p)$ and as a consequence $y_{n}(p) = y_{n-1}(p)= y_{n-2}(p)=... = y_{n-k}(p)$

Now let us prove it for step $n+1$, that is we need to prove that  $y_{n+1}(p) = y_{n}(p) = y_{n-1}(p)= y_{n-2}(p)=... = y_{n-k}(p)$.  According to the rule in ~\ref{..}, $ y_{n+1}(p) = x_{n+1}(p) \neq y_{n-1}(p), ...$ when there exist one $i,j$ so that $ y_{n+1}^{i} \neq  y_{n+1}^{j} $, in this case, according to the rule $i$ does not change its own belief and $ x_i(j) = y_{n+1}^{j}$  or $x_i(j) = y_{n+1}^{j}$. Now we know from the previous iteration that beliefs from $y_{\bar{n}-k} = ... = y_{\bar{n}}$ agree (this is our assumption) and we know as well that $y_{n+1}^{i}$ also agrees with the previous $k$ based on rule\ref{...} (either belief was the same as the previous k or just changed). In this case, we know that all beliefs $y_{\bar{n}-k} = ... = y_{\bar{n}}, y_{\bar{n+1} }$ agree which will lead to a convergence of beliefs (CQFD).  
%\end{proof}
%\end{Theorem}

\hl{if course the convergence is rule dependent and one can want to proof that for a different rule, but this convergence criteria is always good to have because this will as well determine the real-time and efficiency metric of this approach.}


\hl{Selma: i stopped here!}

\paragraph{Beliefs Reduction and Resiliency }
Due to the collaboration and the aggregation function, some autonomous systems adopt the beliefs of others autonomous systems which are more experts, thereby discarding their own belief which disappears from the tree of beliefs (or does not participate anymore to the decision tree). In this case, we are resilient to errors except if experts are making an error. It is clear from the aggregation function that we are resilient to experts $s_{n-1}, s_{n-2}, ..., s_{n-k}$ making an error simultaneously. Where an error can be defined when a belief does not match the ground truth, that is, 

$$y_i(p)\text{ xor } T(p)$$

==> tex/definitions.tex <==
\begin{definition}[Group of Autonomous Systems] 
\label{group}
    A collaborative autonomous system is  defined as a (directed)
    acyclic graph $\mathcal{G}_i = (\mathcal{S},\mathcal{E})$ consisting of a set of vertices or nodes $\mathcal{S}$, where each vertex $s \in \mathcal{S}$ is an autonomous system, as well as of a set of directed edges $\mathcal{E}$. %Each vertex $v \in \mathcal{V}$ is an autonomous system $s \in \mathbb{S}$. 
    %The \textit{start vertex} $v_{start}$ is the first vertex in the application graph and indicates the end-point, on which all jobs of $a_i$ are activated, while the \textit{destination vertex} $v_{end}$ (also an end-point) is the last vertex in the application graph. 
  %  An edge $e=(s_1,s_2) \in \mathcal{E}$ defines a dominance relationship between two autonomous agents $s_1$ and $s_2$ based on the quality of their features. 
     An edge $e=(s_1,s_2) \in \mathcal{E}$ defines belief propagation between two autonomous systems $s_1$ and $s_2$.
      
    % indicates a link which defines a notion of neighborhood between $v_1$ and $v_2$. 
    %We use in the following autonomous systems features to define neighboring relationship between autonomous agents. 
    % \hl{We elaborate more about the notion of neighborhood and how it is defined in the next section.}
    %that during the execution of a job, vertex $v_1$ must be accessed before vertex $v_2$, e.g., computation on a compute node must be performed, before the output data can be communicated over the network.
    
    %\hl{we should refer to a neighborhood of a given node.}
    %https://en.wikipedia.org/wiki/Neighbourhood_(graph_theory)
\end{definition}


 
\begin{definition}[Autonomous System] \label{def:as}
    An autonomous system $s_i = (P_i, \gamma_i)$  is defined by a sphere of its \emph{individual knowledge} $P_i$ and a set of \emph{features}  characterizing the autonomous system. % $s_i$ and a sphere of its \emph{individual knowledge}. %$\kappa_i$. 
    The sphere of individual knowledge $P_i \subseteq \mathcal {P}$ can be defined as a the subset $P_i$ of predicates from a larger set  $\mathcal {P}$ of propositions or predicates characterizing an environmental situation\footnote{An autonomous system can have only local and not a global knowledge about the environment of operation.}. % that can be characterized by a larger set of predicates $\mathcal {P}$ defining a global knowledge about the environment where the autonomous system $s_i$ is operating. %has a belief and based on that 
   % can make a claim. 
\end{definition}


\begin{definition}[ Features and Quality] 
    We define the set $\gamma_i$  of features as a set of parameters or attributes characterizing an autonomous system. Features like sensors quality can be considered as static, their quality does not change (or very gradually) over time. Other features such as distance or perception angle can be considered as dynamic features as they are situation/context dependent and can change over time\footnote{The notion of changes of quality of features over time will not extensively be exploited in this paper. It is mentioned to show that any possible ranking of autonomous systems based on the quality of their features can change over time. For the sake of simplicity, we consider in this paper only one context at a time with a given ranking and not a sequence of contexts where ranking is changing.}. %. They can therefore change relatively "quickly" over time. 
    %{Selma: this idea of expertise we did not exploit it in this paper so i propose to remove it to avoid confusion}  Additional features such as \hl{expertise (find another name)} can depend on the history of previous statements made by the autonomous agent $s_i$.  
    We consider features that are comparable and can be quantified, so that a ranking based on the quality of features can be established. %{Selma: here as well we are not talking at all about the threshold idea in our model} e.g., based on a threshold determining whether the quality of a feature is "good" or "bad".  

    %  (Selma: maybe this bad and good quality we do not need it so far because we did not use it) Features quality is defined according to thresholds which determine whether the quality of a feature is "good" or "bad". A feature $j$ of an autonomous system $i$ has a good quality if it is larger than the threshold $\bar{\gamma_{j}}$,that is 
    %$\gamma_{i,j} \geq \bar{\gamma_{j}} $. 
    
    %  We distinguish between permanent and non-permanent features that we classify as follows,  
    %  \begin{itemize}
    %      \item a set $I_i$ of \emph{inherent} features are permanent and do not change (or very gradually) over time  such as sensors quality.%Selma:maybe in a car someone can upgrade the sensors but not so quickly 
     %   \item a set  $A_i(t)$ of \emph{auxiliary} features that are situation dependent and therefore not permanent, such as perception angle at time $t$ or distance. They can therefore change relatively "quickly" over time,
      %  \item an expertise $E_i((t-\Delta t,t ])$ defined by the history of previous correct statements made by the AS $s_i$ over the interval $\Delta t < t$. \hl{maybe we need the interval eventually, we will see that at the end.}
    %\end{itemize}  
   
    %Trustworthiness can then be defined based on the quality of features.   
\end{definition}



\begin{definition}[Belief]
    A belief of an autonomous system $i$ is a (Boolean) statement on a given proposition (i.e., current situation in the environment). 
    The set of beliefs can be defined as a mapping from the set of autonomous systems $\mathcal{S}$ and the set of environment knowledge predicates $\mathcal{P}$ to the set of Booleans, that is $\mathcal{X}: \mathcal{S}x\mathcal{P} \rightarrow \{True, False\}$. 
    The term $x_i(p)$ defines an initial\footnote{We will see later that an initial assignment can change after belief propagation} Boolean assignment from an autonomous system $s_i \in \mathcal{S}$ about a predicate $p \in \mathcal(P)$ belonging to its sphere of knowledge. 
\end{definition}





\begin{definition} [Belief Aggregation]
    An aggregate function $\odot$ is applied by every autonomous system to form an output belief. The function takes as input an own belief $x_i(p)$  and further beliefs from the selected group of interest $G_i$ to compute an output belief $y_i(p)$ that will further be propagated. Considering a group of interest of size $k$, the aggregate function can be defined as a mapping over the set of Booleans $\mathcal{B}$, so that $\odot: \mathcal{B} x \mathcal{B}^k \rightarrow \mathcal{B}$ %$\odot: \mathcal{B} x \mathcal{B} x...x\mathcal{B} \longrightarrow \mathcal{B}$ 
    for every belief $x_i(p)$ of $i$ and $k$-tuple of beliefs $y_j(p), j \in [1..k]$ from all autonomous systems in $G_i$, 
    an output belief $y_i(p)$ is computed, 
     % $(x_i(p), y_1(p), ..., y_k(p))$ 
    %an output boolean $y_i(p)$
    \begin{equation}
        y_i(p) =  \odot (x_i(p), y_1(p), ..., y_k(p))    
    \end{equation}
    Note that since we deal with Boolean variables, the output $y_i(p)$ is also Boolean and can be either equal to $x_i(p)$ or $\neg x_i(p)$.  
\end{definition}


 A group of interest $G_i$ determines a (sub-)group of $k$ peer autonomous systems that can contribute to forming beliefs for an autonomous system $i$. They can therefore as well contribute to collective decision making for $i$. Every autonomous system $j \in G_i$ belonging to the group of interest has a belief $y_j(p)$ propagated to $i$.

\begin{definition}[Belief Propagation]
    Belief propagation can be defined by applying recursively the belief aggregation function $\odot$ as defined in~\ref{def:belief-aggregation} throughout the binary decision tree. 
    \begin{equation}
        \left\{
            \begin{array}{ll}
             y_j(p) = x_j(p)    \qquad \forall j \in G_{k} 
             \\   
            y_n(p) = \odot (x_n(p), ~ y_{n-1}(p), ~y_{n-2}(p), ..., ~ y_{n-k}(p) )   \qquad \forall n \geq k \\        
            \end{array}
        \right.
    \end{equation}
\end{definition}


% The set of beliefs $x_i$ made by an autonomous system $i$ is defined as a mapping from the set of predicates $P_i$ from the individual sphere of knowledge of $i$ to the set of Booleans
%$P_i \rightarrow \{True, False\}$. A belief $x_i(p)$ is then true or false and constitutes an (internal) assignment from the autonomous system $i$ to the predicate $p \in \kappa_i$. 

%$P_i \rightarrow \{True, False\}$. A belief $x_i(p)$ is then true or false and constitutes an (internal) assignment from the autonomous system $i$ to the predicate $p \in \kappa_i$. 


%\begin{definition}[Individual/Singular Trustworthiness]
%An autonomous agent is defined as trustworthy  (i.e., its claim can be trusted by other autonomous agents) if it has a "good" quality of features. 
%The area of trustworthiness can be defined as the union of all areas where the features are higher than their given respective threshold. $\cup_j~ \gamma_{i,j} \geq \bar{\gamma_{j}} $. 
%An autonomous system is therefore considered trustworthy according to its feature if it falls into the trustworthiness area. That is,  $\forall_j~ \gamma_{i,j} \geq \bar{\gamma_{j}} $

%(Individual)trustworthiness defines whether \emph{one} autonomous system is trustworthy based on its features (i.e., trust the claim made by an AS). % (i.e., trust the claim made by an AS that it will match the ground truth).    

%\end{definition}


%\begin{figure}[h]
%	\centering
 % \includegraphics[scale = 0.25]{tex/figures/individual_trustworthiness_area.png} 
 %\input{tex/figures/features.tex}
%	\caption{Area of (individual\footnote{maybe we can call it agent trustworthiness instead of individual}) Trustworthiness based on Individual Features, View in 2D considering two features.}
 %\label{fig:individual_trustworthiness}
%\end{figure}



==> tex/experiments.tex <==
\section{Experiments and Validation}
\label{sec:exp}

In this section, we discuss experiments and evaluate the proposed concepts of collaborative trustworthiness to increase reliability of autonomous systems using collaboration. For that we generate a number of autonomous systems with different quality attributes. We formulate for every autonomous system multiple different randomly generated individual beliefs.
These latter are then aggregated using different rules to correct collaboratively false beliefs whenever needed using beliefs aggregation and propagation. For that, we construct ordered binary decision trees for beliefs aggregation and propagation where order is defined based on the quality of attributes.  We evaluate using our defined metric of collaborative reliability (see Def., ~\ref{eq:collab-reliab}) the effect of collaboration by varying rules as well as quality of attributes. During the evaluation, we investigate in particular the effect of rules and quality of the group on increasing good decision making, and derive conditions leading to better reliability results under collaboration. In the following, we first detail the considered experimental setup, we later present and analyze experimental results. 

\subsection{Experimental Setup}
We consider an experimental setup similar to the motivating example proposed in Fig.,~\ref{fig:example} where a number of autonomous systems located in a region of interest is randomly generated. We vary the number of of autonomous systems, the quality of attributes and predicates and beliefs to create a set of multiple synthetic benchmarks. 

\subsubsection{Generation of Quality Attributes}
We consider multiple quality attributes for each autonomous system (e.g., distance and perception). Assignment of the quality of attributes to each autonomous system is done randomly in the form of a percentage selected from a uniform distribution between [0..100], where 100\% is the best possible quality for a given attribute\footnote{Note that, since attributes can be quantified differently (i.e., unit of measure of distance is different from sensors quality), we use the interval of selection [0..100] as an abstract uniform representation of a measure of a quality of attributes.}. 
 After generating a set of autonomous systems with different quality attributes, we construct %as shown in Fig. ~\ref{fig:lattice2} 
 a lattice as a partial-order ranking structure. In the absence of a total order between autonomous systems (i.e., non dominance of all autonomous systems based on all quality of attributes), we establish a total order that do not violate the partial order of the lattice, that is an order following a single path of the lattice. 
 

 
 % where autonomous systems with the best quality of attributes are placed at the left and the autonomous systems with the worst quality of attributes are placed at the right of the lattice. 



\subsubsection{Generation of Beliefs} We define multiple different predicates $p_1, p_2, ..., \mbox{etc.}$ (e.g., to model statements such as "an object has been detected") and establish the ground truth as the correct assignment of all considered predicates. We generate randomly for every predicate and every autonomous system beliefs in the form of $0$ (i.e., False) or $1$ (i.e, True). For our synthetic benchmarks and when generating beliefs, we assume that the error rate (i.e, the number of times an autonomous system emits an erroneous belief that does not match the ground truth) of autonomous systems with better quality attributes is lower than the error rate of autonomous systems with worse quality attributes. % Note that the error probability is calculated from the quality of features. 
Therefore, the error rate for every autonomous systems belief is variable and we assume that it can be calculated using a linear factor based on the quality of the attributes. %\footnote{Note that, deriving quality attributes and error rates for specific kind of perception systems, e.g., Lidar sensors requires a careful analysis of the physical characteristics of such sensors and how is perception relates to distance. Since we would like to focus in this paper on the proposed collaborative trustworthiness by applying aggregation and propagation rules, we refer detailed analysis of real perception systems to derive quality of attributes and error rates from realistic systems to future work. }. 

%\hl{@Omar: how was that calculated}) \footnote{\hl{This assumption is a (hidden) assumption which is the base of trust in this paper.}}.  %\hl{@Omar: can we have an example of assignments of attributes and beliefs in the form of a table?} In table ~\ref{tab:benchmark-example-table}, we can see an example of how a synthetic benchmark consisting of four agents is formalized consisting of each agent's belief and quality of attributes.


Table ~\ref{tab:benchmark-example-table} provides an example of random assignments of quality of attributes and beliefs following the example in Fig,~\ref{fig:lattice}. Note that, deriving quality attributes and error rates for specific kind of perception systems, e.g., Lidar sensors requires a careful analysis of the physical characteristics of such sensors and how is perception quality relates to distance. Since we would like to focus in this paper on the proposed model for collaborative trustworthiness by applying aggregation and propagation rules, we refer detailed analysis of real perception systems to derive quality of attributes and error rates from realistic systems to future work. 

%\hl{@Omar: use the terminology synthetic benchmarks when talking about synthetic benchmarks.}

%\hl{@Omar: also a terminology thingy, maybe its better to use context instead of situation and then iterations or something else for every contexts }

\subsubsection{Considered Rules}
We evaluate our setup considering multiple aggregation rules, namely, the "n-experts" rule with the following variants: the "Most Expert", "Two Experts", "Three Experts", "Fours Experts", in addition to the  "Majority", and "Gravity Point" rule defined below. The "n-expert", "Most Expert" and "Majority" are as defined in Sec.~\ref{sec:rule-definitions}. The "Gravity Point" rule considers, similarly to the majority rule, beliefs from both autonomous systems with better and worse quality of attributes. However, it considers, unlike the majority rule, only a subgroup is considered as the group of interest and not all the set of autonomous systems. By considering quality of attributes and their ranking, the considered autonomous system constitutes the gravity point of the group of interest. 
For a given autonomous system (e.g.,in the motivating example a vehicle), the group of interest is composed first of one autonomous system with a higher quality of attributes and another autonomous system with a lower quality of attributes. In case of peer disagreement, change of belief occurs when both autonomous systems in the group of interest have a consensus (i.e., similar beliefs that contradict with the considered autonomous system). When one autonomous system (of better or worse quality of attributes) agree with the belief of the considered autonomous system and the other disagrees, the group of interest is expanded iteratively considering an additional autonomous with better quality of attributes and another autonomous system with lower quality of attributes, the considered autonomous system where belief aggregation occurs still remain as the gravity point of its group of interest. % where the vehicle of interest constitutes the gravity point of the formed group. 
When the group extends, the majority rule within the group of interest is applied to determine a possible change of belief as a result of beliefs aggregation and after that propagation\footnote{Note that, any rule can be applied for aggregation. The rationals behind investigating the gravity rule is to investigate a rule which can be seen as a compromise between the n-experts variant rule considering only autonomous systems with a better quality of attributes (i.e., more trustworthy) and that can be still subject to introduced errors when all experts result simultaneously in erroneous beliefs, and 
the majority rule considering the entire set of autonomous systems including all autonomous systems with lower quality of attributes (i.e., less trustworthy).}. % and the n-experts variant rule considering only autonomous systems with a better quality of attributes (i.e., more trustworthy). % to form for decision making for each vehicle with a given level of trustworthiness (determined by quality of its attributes), a reasonable subgroup with better and lower levels of trustworthiness to detect possible errors. }. 

\input{tables/benchmark-example-table}



%: voting was also done however, only a subgroup of vehicles were the ones voting. This subgroup of vehicles was set to be one vehicle higher in quality of features than the vehicle of interest, and one lower. Afterward, voting was done between these two vehicles and if there was consensus, then the belief was propagated. If there is no consensus, the subgroup of vehicles is increased by one vehicle in each direction to perform voting again and so forth until a belief is voted more than the other and then propagated.

  
%\begin{itemize}
%    \item The "n-expert" rules: the previous ‘n’ vehicles that were best in the quality of features, formed our subgroup of interest as discussed in definition \ref{group} and their beliefs [0, 1] about whether there was an object detected or not, were the ones that were propagated.
 %   \item The "Majority" rule: voting was done and the beliefs propagated were the most voted beliefs.
 %   \item The "Gravity Point" rule: voting was also done however, only a subgroup of vehicles were the ones voting. This subgroup of vehicles was set to be one vehicle higher in quality of features than the vehicle of interest, and one lower. Afterward, voting was done between these two vehicles and if there was consensus, then the belief was propagated. If there is no consensus, the subgroup of vehicles is increased by one vehicle in each direction to perform voting again and so forth until a belief is voted more than the other and then propagated.
%\end{itemize}




%\begin{figure}[H]
%\centering
%\includegraphics[width=0.5\textwidth]{figures/Experimental Setup.png}
%\caption{Experimental setup used in a region of interest where a group of autonomous vehicles with different quality of features approach a person and each flag a belief whether there is a person detected or not}
%\label{fig:exp_setup}
%\end{figure}



\subsection{Effect of the Rules on Collaborative Reliability}
In the first series of experiments, we use synthetic benchmarks generated considering 20 autonomous systems and two attributes and their qualities.  We generate for every autonomous system randomly, as explained in the previous section, beliefs based on autonomous systems quality of attributes. 
For the same example with a given number of autonomous systems and same quality of attributes, we generate multiple \emph{iterations}, each iteration constitute an assignment of beliefs. 
%With randomly generated qualities as explained , and \h{number of vehicles and quality of features} beliefs assignment based on the quality of attributes for each agent. 
We apply for every iteration aggregation rules and propagation. In order to obtain sound comparisons between the applied rules, the same generated example is used for each rule to observe the effect of rules when using the collaboration on both errors correction (i.e., number of corrected errors) and error creation (i.e., number of introduced errors). We generate up to 100 different iterations \hl{maybe use example} for the synthetic benchmark with 20 autonomous systems, results on the percentage of errors are summarized in Fig.~\ref{fig:errors_aft_coll_high_quality}. 


Individual errors are errors resulting from the quality of attributes of each autonomous determining a given error rate. Individual errors characterize the level of reliability (before the collaboration) that we aim to improve with the collaboration and is used  as a baseline for comparison when applying beliefs aggregation and propagation rules. 
As observed in Fig.~ \ref{fig:errors_aft_coll_high_quality}, for the considered examples, the percentage of the sum of all individual errors over 100 iteration before collaboration is depicted (52.7\%). This percentage shows all errors from autonomous systems when assigning beliefs (without collaboration) randomly following the error rates over the 100 iterations.  Applying each rule leads to number of introduced errors and a number corrected ones. Percentages of the sum of introduced and corrected errors over all 100 iterations for each rule are depicted in Fig.~\ref{fig:errors_aft_coll_high_quality}. 
We overall observe that by applying the rules, the number of corrected errors is increased by using the collaboration to reach the best values with the most expert and the 2-experts rule. Both as well lead to a small number of introduced errors. 

We observe that the most-expert rule allows to introduce a relatively small percentage (1.7\%)  of errors compared to the majority rule (17.25\%). The most-expert rule allows as well to introduce a large percentage of corrected errors (50.4\%) compared to the majority rule (24.95\%). We also observe that overall the two-experts rule outperforms all other rules resulting in the minimum percentage of introduced errors (0.55\%) and maximum percentage of corrected errors after beliefs propagation (50.8\%). The 2-experts rule has nearly similar performance compared to the most-expert rule when it comes to corrected percentage of errors. However, the percentage of introduced errors is higher in the case of the most-expert rule, having a 1.15\% difference. Indeed in the n-expert rule, errors are introduced if all experts make simultaneously an error. Therefore the 2-expert rule is more robust compared to the Most-expert rule as both experts have to make errors simultaneously which is less likely to happen compared to one expert. The "3-expert" and the "4-expert" rules have similar but higher percentages of introduced errors, however, the error correction is lower than the two-expert rule (46.7\% for the three-expert rule and 33.35\% for the four-expert rule). Therefore, the higher the number of experts taken into account for belief propagation, the more resilient the group is to change the beliefs of its members, as for an autonomous systems to change its belief, all n-experts should have consensus and that might not happen so often for a high number of experts as seen in the three-expert and four-expert rules. 



\input{tex-figures/errors_aft_coll_high_quality}

The Majority rule, as it can be observed, lead to very high percentage of introduced errors (17.25\%), and the lowest percentage of corrected errors (24.95\%), and this is due to the rules' nature, as the output of the voting between autonomous systems heavily depends on the quality attributes of the entire group forming the set of autonomous systems. The higher is the quality of attributes of autonomous systems in the group and the better the output of the majority rule, otherwise the rule can lead to poor results in terms of errors correction when using the collaboration. A detailed discussion about how the quality of the group influences collaborative reliability is presented in the next section. 

%, however, a high-quality group is very rare to find in the environment and is a plausible reason to not rely on this rule. 

The Gravity-Point rule is similar to the Majority rule in terms of percentage of corrected errors (25.6\%) as it applies the same concept of voting, yet the voting takes place between the closest (based on the quality of attribute) autonomous system  to the autonomous system where aggregation is performed, and that maintains the level of quality for the autonomous system voting resulting in a low percentage of introduced errors (0.7\%). However, for the less trustworthy autonomous system (with lower quality of attributes), the output of the sub-group voting is also determined by the quality of the sub-group, and that may results in degraded results during beliefs propagation.

%and that discloses to us that the higher the number of experts taken into account for belief propagation, the more resilient the group is to change the beliefs of its agents, as for an agent to change its belief, the n-higher experts should have consensus and that might not happen so often for a high number of experts. 
 



%the Two-expert rule outperformed all, resulting in the least introduced errors and the most corrected errors after the belief propagation. The Most-expert rule might have a close number of corrected errors, but with more introduced errors than the Two-expert rule and that concludes that the Two-expert rule is more robust to an expert making an error than the Most-expert rule. The Three-expert and the Four-expert rules have similar but higher introduction of errors, however, the error correction is far lower than the Two-expert rule, and that discloses to us that the higher the number of experts taken into account for belief propagation, the more resilient the group is to change the beliefs of its agents, as for an agent to change its belief, the n-higher experts should have consensus and that might not happen so often for a high number of experts. 


% \begin{figure}[H]
% \centering
% \includegraphics[width=0.7\textwidth]{figures/Individual Errors, Introduced Errors and Corrected Errors for all Rules_high_quality.png}
% \caption{Individual errors before belief propagation, and corrected and introduced errors after belief propagation are shown for each rule. The lower the introduced errors after belief propagation the better, and the higher the corrected errors the better.}
% \label{fig:errors_aft_coll_high_quality}
% \end{figure}


\subsection{Effect of the 
Quality of the Group on Collaborative Reliability}
In a second series of experiments, we investigate 
% Another set of experiments were investigated, where the experimental interest is to compare 
the effect of the quality of attributes of the group on the number of errors introduced and errors corrected after applying beliefs aggregation and propagation rules with the collaboration.  
%error percentages.

\subsubsection{Generation of Different Quality of Groups} As discussed previously, the quality of attributes affects the errors rate of an autonomous system when forming a belief (i.e., the higher is the quality of attributes, the lower is the error rate). We generate two synthetic benchmarks of 20 autonomous systems each, and each synthetic benchmark is composed of a group with different quality of attributes, see Fig.~\ref{fig:sum_errors}. In the first group all (or most) autonomous systems have a high quality of attributes, and in the second group all (or most) autonomous systems have a poor quality of attributes. 
We generate as previously for every benchmark beliefs over 100 different iterations with an error rate based on the quality of attributes. 
 %(\hl{@Omar: we need to be clear what is a scenario and what is an iteration, also what how many vehicles were considered in the figures?}). 
 %We generate for every synthetic benchmark beliefs based on their attributes quality for 100 different iterations, and % for the two different groups based on that criteria and 
The sum of all individual errors %\hl{@Omar: is it now a percentage or not} 
before the collaboration based on the results are depicted in Fig.~\ref{fig:sum_errors_aft_coll_low_quality} for the low-quality group, and Fig. ~\ref{fig:sum_errors_aft_coll_high_quality} for the high-quality group. We observe the sum of errors performed by all autonomous systems ranked from the higher to the lower experts. We notice that the group of vehicles with higher quality attributes (Fig.~\ref{fig:sum_errors_aft_coll_high_quality}) make less errors than the group formed by autonomous systems with lower quality attributes (Fig.~\ref{fig:sum_errors_aft_coll_low_quality})  %(\hl{@Omar: whenever possible, please fix the figures numbers in the caption and also in the text.}). 




 
 % In Fig.~\ref{...} the number of errors per vehicle is depicted, vehicles are ranked based on their quality of attributes. Therefore, the number $1$ in the x-axis corresponds to the number of errors that the most-expert has performed. We notice that for every group, the number of errors for every vehicle is increasing with the raking of expertise.  Overall the sum of errors over 100 iterations performed by the group with higher quality of attributes is less than the group with lower quality of attributes (\hl{@Omar: how much? can we normalize this as it is not also clear what is 5 errors over a max of 80 errors or 100 iteration}) .% The sum of errors performed by the experts over a 100 iterations was far lower (\hl{@Omar: how much? can we normalize this as it is not also clear what is 5 errors over a max of 80 errors or 100 iteration}) as the number of experts increased.
 
Similarly, we further generate multiple groups with different attributes quality, see Fig.~\ref{fig:diff_groups_dist}, that results in different errors distributions, and each group is generated independently by varying the quality of attributes of its members. Dist.1 shows that the entire group has poor quality and can therefore benefit less from the collaboration and Dist.4 has a group with a high quality of attributes, therefore applying collaboration on that group would have positive effects. %\hl{@Omar: maybe we can characterize this by the median or so} 

 \input{tex-figures/sum_errors_aft_coll_high_quality}

\input{tex-figures/diff_groups}


\subsubsection{Effect on Collaborative Reliability}
We investigate the effect of collaboration through beliefs aggregation and propagation using the previously defined rules over all four different groups with different distributions of quality of attributes. The goal is to increase reliability collaboratively and to increase the number of corrected errors while decreasing the number of introduced errors. We quantify results using the previously defined metric \emph{Collaborative Reliability} (in Eq.,~\ref{eq:collab-reliab}). For further clarification, the effect of the quality of the groups on the collaborative reliability ratio is shown in Fig.\ref{fig:col_reliability_2_exp_low_quality}, where the ratio is output to two different groups, a high-quality one and a low-quality one. Results are shown for all 100 iterations. 

\input{tex-figures/col_reliability_2_exp_low_quality}

% \input{tex-figures/diff_groups}

Note that according to the d
efined collaborative reliability metric, when the number of introduced errors and corrected errors is the same then the collaborative reliability ratio is equal to $R_i^c = 1$. The goal is as described previously: increase the number of corrected errors while minimizing the number of introduced errors. When all errors are corrected and no error is introduced, then the collaborative reliability ratio is optimally equal to $R_i^c = 0.5$. This is the case for the group of autonomous system with a high quality of attributes distribution (see Fig.~\ref{fig:col_reliability_2_exp_low_quality}) Inversely, when the number of introduced errors is higher than the number of corrected errors then $R_i^c \geq 1$ as it is the case in the group of autonomous systems with low quality of attributes. Results are further summarized for the four groups with different qualities are summarized in Fig.~\ref{fig:col_reliability} where comparison between the groups is performed after applying all the rules.




\input{tex-figures/col_reliability}

It can be observed in Fig.~\ref{fig:col_reliability}, for Distribution 1, the error distribution is the highest (ranging from 80\% to 95\%) resulting in an average collaborative reliability that is always above 1, along with Distribution 2, which has below-average quality of features (having an error distribution of 26\%-90\%). For these distributions, the average introduced errors is more than the average corrected ones resulting in the shown average Collaborative Reliability metric for all the rules in Fig.~\ref{fig:col_reliability}. For Distribution 3, the groups' error distribution is evenly distributed as the group had autonomous systems making a low number of errors, and also autonomous systems making an error of almost 64\%. This error distribution successfully develop a system where an even hierarchy can be obtained, which is what we observe in any system in our environment, and Distribution 3 greatly resembles a real-life autonomous system where there is an acceptable range of errors that can be made by autonomous systems. In this distribution, it can be observed that the performance is best-of-all for the Two-Expert rule having an average Collaborative Reliability of almost 0.5, which means that almost all the individual errors before belief propagation are changed to corrected errors after belief propagation resulting in a 0.5 collaborative reliability. It can also be observed that the Most-Expert and Three-Expert rules have a much better performance in this group than the others meaning that the quality of the group greatly affects the resulting collaborative reliability. For Distribution 4, the groups' quality of features are the best resulting in a range of errors 0-22\%. The results of this group are greatly similar to the results of the hierarchy group (3), where the differences in the average ratios are very low as seen in Fig.~\ref{fig:col_reliability}. However, the performance of the Two-Expert rule in the hierarchy group (3) still outperformed all the other rules and groups, which is greatly advantageous as this group is the most resembling a realistic diverse group. Also, it can be observed that for the high-quality group (4), the Majority rule and the gravity point rule outperform the Two-Expert rule as the error probability is much lower for this group, and voting results in better output propagation than the hierarchy group (3).

\hl{Selma: i stopped here}

 
%The output Collaborative Reliability is computed using the equation defined in Sec.~\ref{sec} \hl{xx}, where the fraction indicates the ability of the group to collaboratively increase their reliability or not. This is achieved by having a lower output, as when the output fraction decreases, that indicates that the corrected errors are more than the introduced errors in the fraction \hl{@Omar: here you talk about lower output, is it nominator and denominators?}. Results are summarized in Fig.~\ref{fig:errors_aft_coll_high_quality }. 

%The quality of the group affects the quality of the output of the Collaborative Reliability significantly as briefly observed before. To further explain this effect, 100 iterations of synthetic benchmarks were computed and the output of the groups was examined. This experiment was done twice, once with a group having an average of high-quality features and another with a group having a low average-quality feature.




% \begin{figure}[H]
% \centering
% \includegraphics[width=0.7\textwidth]{figures/Sum of Errors Performed by Experts in a synthetic benchmark for 100 Iterations Following Random Error Assignment .png}
% \caption{Sum of Individual errors performed by Experts after belief propagation over 100 iterations by a low-quality features group. The low-quality features group results in a higher sum of errors than the high-quality features group see Fig.\ref{fig:sum_errors_aft_coll_high_quality}}
% \label{fig:sum_errors_aft_coll_low_quality}
% \end{figure}


% \begin{figure}[H]
% \centering
% \includegraphics[width=0.7\textwidth]{figures/Sum of Errors Performed by Experts in a synthetic benchmark for 100 iterations(Error Probability increment).png}
% \caption{Sum of Individual errors performed by Experts after belief propagation over 100 iterations by a high-quality features group. The high-quality features group results in a lower sum of errors than the low-quality features group see Fig.\ref{fig:sum_errors_aft_coll_low_quality}}
% \label{fig:sum_errors_aft_coll_high_quality}
% \end{figure}

% To further show the effect of the quality of the groups on Collaborative Reliability, the results of each rule can be observed in Fig. \ref{fig:col_reliability}. These results were evaluated for different groups with different quality features, and these groups can be observed in Fig. \ref{fig:diff_groups}. 


% \begin{figure}[H]
% \centering
% \includegraphics[width=0.7\textwidth]{figures/chart2 with line.png}
% \caption{Average Collaborative Reliability for Different Groups and Different Rules. For each generated group, the rules were applied, belief propagation occurred, and the results were shown. For each rule and each group, depending on the group's error distribution, the average collaborative reliability is calculated, and the lower the average collaborative reliability ratio, the better.}
% \label{fig:col_reliability}
% \end{figure}





% \begin{figure}[H]
% \centering
% \includegraphics[width=0.7\textwidth]{figures/Col_Rel_2_Exp_Bel_Avg_&_High_Quality_scatter.png}
% \caption{Collaborative Reliability Ratio behavior of Two-Expert Rule for the high-quality and low-quality group. It can be observed that the ratio for the low-quality group is always above 1 resulting in a high Collaborative Reliability Ratio average and the high-quality group has an average of 0.5 Collaborative Reliability Ratio reflecting the low error probability of the group.}
% \label{fig:col_reliability_2_exp_low_quality}
% \end{figure}

\subsection{Key Takeaways and Discussion}

As observed in the previous sections, the Two-Expert rule has higher performance than all the other rules, and that is due to the fact that it is more resilient than the Most-Expert rule, more flexible to change than the Three, and Four-Expert rules, and relies on better judgment than the Majority, and the Gravity-Point rules. 

The quality of the group is of very high importance to investigate also, as when experimented, it shows that the higher the quality of features a group possesses, the better the output of Collaborative Reliability. Also, output data shows that it is better to rely on two experts rather than one in order to have better output collaborative reliability.


%\paragraph{\textbf{Discussion: Rule for Group Selection}}
%\begin{definition}[Rules for Group Selection]
%In order to illustrate the concept of rules, we consider in the following very simple and straightforward set of rules for belief propagation that can be applied, and discuss that, when applied, these latter do not necessarily lead to a collectively increased reliability.

%\begin{itemize}
%    \item "Most Expert" rule
%In the most expert rule, the belief (e.g., an object has been detected) of the most "expert" autonomous system is propagated to the rest of the group, see Fig.~\ref{fig:rules}-(a). Each member of the group systematically adopts the belief of the most expert autonomous system, even if contradicting with own belief (e.g., an object has not been detected) or beliefs from other autonomous systems. The rule builds on trusting the opinion of the most expert, %(which is the most trustworthy in the group based on the quality of its feature)
%as it constitutes the autonomous system which has the best quality of features in the group and which thereby considers its belief as the most trustworthy. This rule considers that only the most expert is responsible of forming a correct belief. However, one weakness of the rule is that it relies on \emph{one} single opinion and is therefore not resilient to the case where the most expert autonomous system makes an error of judgement. 

%$$ \forall~~ s_i, G_i = \{s_{sup}\}$$ \hl{i think if we consider that the higher is the better .. todo check that..}

%\item "n-expert" rule, 
%it is $n$ of those who have better features, \hl{todo: give an example of 2-expert rule.}
%$$ \forall~~ s_i, G_i = \{s_1, s_2, ... s_n\} \text{so that } s_1 > s_i, s_2 > s_i \text{ and } s_n > s_i
%$$

%\item "Majority" rule
%In the majority rule, beliefs from all autonomous system are propagated to the rest of the group. Each autonomous systems therefore collects all beliefs including own belief and adopts the belief of the majority of the group similar to a voting mechanism, see Fig.,~\ref{fig:rules}-(b). In this case, all autonomous systems in the group are responsible of forming a correct belief. While this approach offers a given notion of fairness as all beliefs are considered, this can as well constitute the main weakness of the approach. Indeed, the majority rule considers all beliefs in the group including beliefs from less experts autonomous systems with a low quality of features. In this case all autonomous systems, including less trustworthy ones contribute to forming a correct belief. In the smart intersection example considered previously, even vehicles with a larger distance from the pedestrian or with a bad perception angle will contribute to the overall decision making process, thereby possible leading to an error in the propagated belief and overall decrease in reliability when using the majority rule for collective reasoning. 

%\hl{here mention that the group of interest for every autonomous system  is the entire set }
%$$ \forall~~ s_i, G_i = \mathcal{S}$$ 

%\end{itemize}
 
%\end{definition}

%\paragraph{Peer Disagreement} Peer disagreement occurs whenever two autonomous systems $(i,j)$ have different beliefs about the same proposition $p$, that is \hl{Maybe here define peer disagreement with a condition of having at least 3 autonomous systems in the environment}
%$$\exists(i,j) ~~\mbox{s.t.,} ~~x(i) \neq y (j)$$


\hl{add the fact that we can do either a direct ordering or an ordering based on the regions, which allows a more detailed ranking coz we know how much we are better which is the maximum box size. In this case what we are ranking are regions and then we do a mapping between the region and the autonomous systems themselves. }



\hl{TODO: check using the results of leslie lamport that no agreement can be found in the presence of at least n = 3m+1 or greater of systems if m of them are faulty, it means that in the quality of our system, if one third of the population have errors or more then we will definitely decrease our collaborative reliability. }

==> tex/formalization.tex <==
%\section{Model of Computation for Collaborative Trustworthiness}
%\hl{5 pages}
%\label{sec:moc_model}


\section{Peer Disagreement, Beliefs Aggregation and Propagation}

However, one of the main issues in the epistemic sense is to deal with \emph{peer disagreement}. That is, should an individual (or a system) adjusts an own belief based on additional knowledge, which can as well be contradictory, provided by other peers? In the following, we discuss how similar principles can be applied to autonomous systems.
\hl{todo: emphasize the problem of peer disagreement}

\subsection{Peer Disagreement and Beliefs Aggregation}
As mentioned previously, every autonomous system $i$ has an own belief $x_i(p)$ on a given proposition $p$. It receives as well beliefs $y_j(p)$ from other autonomous systems $j \in G_i$ belonging to a group of interest $G_i$ that we will define more precisely in the following. 

%\begin{definition} [Peer Disagreement]
\paragraph{Peer Disagreement}
Peer disagreement occurs whenever two autonomous systems $(i,j)$ have different beliefs about the same proposition $p$, that is
$$\exists(i,j) ~~\mbox{s.t.,} ~~x(i) \neq y (j)$$
%\end{definition}



\begin{definition} [Aggregation Rules]
The aggregation function can be defined in multiple ways. The goal of the aggregation function is to reduce peer disagreement, by adopting the beliefs of other autonomous systems when they disagree with own belief. Several aggregation rules can be defined, we use in the following the following simple aggregation function, 

%$$\odot = x_i(p) \land \neg y_1(p), ..., \neg y_k(p) \longrightarrow \neg x_i(p) $$

%$$
%\sigma(s,i) = \left\{
%    \begin{array}{ll}
%        \tau_{si} & \mbox{si } \{s,i\} \in E \\
%        \infty & \mbox{sinon.}
%    \end{array}
%\right.
%$$

$$
y_i(p) = \odot (x_i(p), ~~\forall j\in G_i~y_i^j (p) )= \left\{
    \begin{array}{ll}
        \neg x_i(p) & \mbox{if } x_i(p) \land \neg y_i^1(p)\land ...\land \neg y_i^k(p) \\
         x_i(p) & \mbox{otherwise.}
    \end{array}
\right.
$$

According to this rule, an autonomous system $i$ changes its own belief on a proposition $p$,  $x_i(p)$ when this latter disagrees with all input beliefs $y_j(p)$ belonging to the group of interest for $i$, $G_i$. 

Note that by changing own belief, \hl{this is the arithmetic equal, i am not sure if we should not write it in the boolan sense.}
$$y_i(p) = y_i^1(p)\land ...\land \neg y_i^k(p)$$
\end{definition}




\begin{definition}[Rules for Group Selection]
In order to illustrate the concept of rules, we consider in the following very simple and straightforward set of rules for belief propagation that can be applied, and discuss that, when applied, these latter do not necessarily lead to a collectively increased reliability.

\begin{itemize}
    \item "Most Expert" rule
In the most expert rule, the belief (e.g., an object has been detected) of the most "expert" autonomous system is propagated to the rest of the group, see Fig.~\ref{fig:rules}-(a). Each member of the group systematically adopts the belief of the most expert autonomous system, even if contradicting with own belief (e.g., an object has not been detected) or beliefs from other autonomous systems. The rule builds on trusting the opinion of the most expert, %(which is the most trustworthy in the group based on the quality of its feature)
as it constitutes the autonomous system which has the best quality of features in the group and which thereby considers its belief as the most trustworthy. This rule considers that only the most expert is responsible of forming a correct belief. However, one weakness of the rule is that it relies on \emph{one} single opinion and is therefore not resilient to the case where the most expert autonomous system makes an error of judgement. 

$$ \forall~~ s_i, G_i = \{s_{sup}\}$$ \hl{i think if we consider that the higher is the better .. todo check that..}

\item "n-expert" rule, 
it is $n$ of those who have better features, \hl{todo: give an example of 2-expert rule.}
$$ \forall~~ s_i, G_i = \{s_1, s_2, ... s_n\} \text{so that } s_1 > s_i, s_2 > s_i \text{ and } s_n > s_i
$$

\item "Majority" rule
In the majority rule, beliefs from all autonomous system are propagated to the rest of the group. Each autonomous systems therefore collects all beliefs including own belief and adopts the belief of the majority of the group similar to a voting mechanism, see Fig.,~\ref{fig:rules}-(b). In this case, all autonomous systems in the group are responsible of forming a correct belief. While this approach offers a given notion of fairness as all beliefs are considered, this can as well constitute the main weakness of the approach. Indeed, the majority rule considers all beliefs in the group including beliefs from less experts autonomous systems with a low quality of features. In this case all autonomous systems, including less trustworthy ones contribute to forming a correct belief. In the smart intersection example considered previously, even vehicles with a larger distance from the pedestrian or with a bad perception angle will contribute to the overall decision making process, thereby possible leading to an error in the propagated belief and overall decrease in reliability when using the majority rule for collective reasoning. 

\hl{here mention that the group of interest for every autonomous system  is the entire set }
$$ \forall~~ s_i, G_i = \mathcal{S}$$ 

\end{itemize}
 
\end{definition}

\subsection{Structuring Beliefs and Beliefs Propagation}

\hl{-->}
We models beliefs as boolean variables. Therefore, for every autonomous system, a boolean variable represent a belief on a given proposition, e.g., “an object has been detected”. We further use Binary Decision Diagrams (BDDs) to model all possible beliefs from all autonomous systems referring to a given proposition. Fig~\ref{fig:bdd_example} depicts an example with 3 autonomous systems. Every vertex is a boolean variable representing the belief of one autonomous system, every vertex has two arcs, either the belief is assigned 1 (true) or assigned 0 (false). Each terminal vertex is labelled 0 or 1 which corresponds to the belief of the \emph{last} autonomous system. 

\hl{>--}


\begin{figure}
	\centering
  \includegraphics[scale = 0.45]
{figures/BDDs_example}
	\caption{Binary Decision Diagram (BDD) considering 3 autonomous systems.  Decision variables for autonomous system are ranked from the most expert to the least expert one. }
	\label{fig:bdd_example}
\end{figure}


Given a proposition $p$\footnote{Note that we consider so far and for the sake of simplicity, one BDD per proposition $p$}, every autonomous system $i$ believes that $p$ is true or not, that is $x_i(p)$ or not $\neg~ x_i(p)$. The set of all possible beliefs for a group of autonomous agents can be structured and modeled using Binary Decision Diagrams (BDDs)~\cite{bdds-seminal}. 


\begin{definition}[Beliefs as BDDs]
Beliefs about a given proposition are modeled as directed acyclic graphs with labeled nodes and edges as follows, 
\begin{itemize}
    \item there are two types of nodes: decision nodes and terminal nodes. 
    \item every decision node is labeled $x_i(p)$ and has two outgoing edges, one edge is labeled by 0 for \emph{false} and another is labeled 1 for {true}.
    \item a terminal node is labeled by either 0 or 1 and has no outgoing edge. A terminal node is called a 0-terminal or a 1-terminal node according to its label. 
\end{itemize}
\end{definition}

\paragraph{Ordering of Beliefs}
We consider a given order of variables in the BDDs, where for each node   $x_i(p)$ < $x_j(p)$. The order we consider should follow an order in the lattice, that is
\hl{todo: say that all variables in the BDD should satisfy this condition}
$$s_i> s_j \implies x_i(p) < x_j(p) $$
In this case, beliefs in the binary decision digram can propagate from the most expert to the least expert autonomous system according to the established lattice order. 
Terminal nodes then contain the beliefs of the \emph{last} node. 

\begin{definition}[Order of variables and group of interest]
%\hl{to define this in a recursive way we need to assume that the part of the group to which belongs the group of interest is following the experts and therefore the orders, }
We define for an autonomous system $i$, the group of interest as the set of beliefs of $k$ autonomous systems whose quality of features is better than $i$, that is $$s_i \leq \{s_{i-1}, s_{i-2}, ..., s_{i-k}\}$$
%$$G_i = \{y_{n-1}(p),~ y_{n-2}(p), ~..., ~y_{n-k}(p)\}$$ 
The set of corresponding beliefs from the defined group of interest can therefore be described as follows, 
%$$G_i = \{y_{i}^{i-1}(p),~ y_{i}^{i-2}(p), ~..., ~y_{i}^{i-k}(p) \}$$ 

$$G_i = \{y_{i-1}(p),~ y_{i-2}(p), ~..., ~y_{i-k}(p) \}$$ 


%These latter will contribute to building the beliefs 
%$$y_i (p)$,
\end{definition}




%\begin{definition}[Belief Propagation]
\paragraph{Belief Propagation}
Belief propagation can be defined by applying recursively the belief aggregation function $\odot$ as defined in~\ref{def:belief-aggregation} throughout the binary decision tree. 
%\end{definition}

\begin{equation}
\left\{
    \begin{array}{ll}
     y_j(p) = x_j(p)    \qquad \forall j \in G_{k} 
     \\   
    y_n(p) = \odot (x_n(p), ~ y_{n-1}(p), ~y_{n-2}(p), ..., ~ y_{n-k}(p) )   \qquad \forall n \geq k \\        
    \end{array}
\right.
\end{equation}


%\hl{belief propagation is about applying the aggregation rule recursively on the set of variables of the beliefs of autonomous systems. The goal is also to minimize peer disagreement through propagation}


%\hl{Belief propagation is a recursive function..}
%\hl{-----Selma: i sopped here, i am fixing notation using the bot symbol as well}
%$$
%\odot (x_i(p), \forall j\in G_i,~y_i^j (p) )= 
%\left\{
%    \begin{array}{ll}
%       % y_1(p) = x_1(p) \\
%       y_1(p) =  \odot (x_1(p), ~\bot, ..., \bot)} = x_1(p) \\
%        y_2(p) = x_2(p) \\
%        ... \\
%         y_k(p) = x_k(p) \\
%         ~  \\
%        % y_n(p) = \odot (x_n(p), \forall j\in G_i,~y_i^j (p) )
        
% y_n(p) = \odot (x_n(p), ~ y_{n-1}(p), ~y_{n-2}(p), ..., ~ y_{n-k}(p) )
         
%       % \neg x_i(p) & \mbox{if } x_i(p) \land \neg y_i^1(p)\land ...\land \neg y_i^k(p) \\
%       %  x_i(p) & \mbox{otherwise.}
%    \end{array}
%\right.
%$$

\hl{-->}
Every autonomous system receives beliefs from other autonomous systems belonging to a group of interest that can be defined based on different rules or procedures. When for example the majority rule is used, the group of interest correspond to all autonomous systems.  When an expert-based rule is used, then the group of interest refers to a (sub)set of experts. A more detailed definition will be presented in Sec.~\ref{sec:moc_model}. Every autonomous system can change its own belief after applying an aggregate function. The goal of the aggregate function is to reduce peer disagreements where an autonomous system can change its own belief to adopt the belief of the rest of the group of interest, i.e., for instance the opinion of more experts nodes. Fig~\ref{fig:aggregate_function} depicts an example of such aggregate function under peer disagreement. In this case the autonomous system $i$ changes its belief when this latter disagrees with all beliefs from other autonomous systems belonging to the group of interest. 

By reducing peer disagreement and adopting the beliefs of other autonomous systems when they contradict with own belief, we aim at reducing errors (e.g., from one autonomous system perception system) by relying on beliefs from other members of the group. The goal is to therefore increase reliability collaboratively. Note that by adopting the belief of other members of the group, an autonomous system is generally resilient to errors except for the case when multiple members of the group of interest are making errors simultaneously. A more detailed discussion regarding the choice of the group of interest, the aggregation rule and reliability will be presented in Sec.~\ref{sec:moc_model}.



\begin{figure}
	\centering
  \includegraphics[scale = 0.45]
{figures/aggregation}
	\caption{Example of an aggregate function for belief aggregation. The function considers $k$ input beliefs $y_j(p)$ on a proposition $p$.  Belief of a node $x_i(p)$ is changed if there is a disagreement with all input beliefs.}
	\label{fig:aggregate_function}
\end{figure}
\hl{>--}

\subsubsection{Belief Propagation and Transformation Rules}

\hl{-->}
The adopted order of variables in the BDDs structure follows a total order from the lattice. In this case, belief propagation in the BDDs starts from the most expert to the least expert node (or autonomous system). The aggregation function is then used by every node in the BDD to decide whether the autonomous system changes its own belief to adopt the belief of the most expert one(s). The aggregated belief is further propagated and contributes to later beliefs aggregation. 

Belief aggregation and propagation lead to a transformation of the BDD to a simpler form as depicted in Fig.~\ref{fig: ....}, where less experts adopt the belief of the most expert one (s). In that case terminal vertices correspond to the belief of the last autonomous system(s). which allows to reduce as well the complexity of systems. 


\hl{at the end of this section say that the following sections will present a detailed model and formalization of this and that the experimental section will evaluate x and y.}

\begin{figure}
	\centering
  \includegraphics[scale = 0.45]
{figures/BDDs_Reduction}
	\caption{(a): non reduced BDDs, (b): reduced BDD considering the most expert rule, (c) reduced BDD considering the 2-experts rule.}
	\label{fig: ...}
\end{figure}

\hl{>--}

We define transformation rules over the defined BDD graphs to reflect belief aggregation and propagation and which will lead to a transformation and reduction of the BDD graphs. 

\begin{enumerate}
    \item Remove duplicate terminals: eliminate all but one terminal vertex with a given label and redirect all arcs into the eliminated vertices to the remaining one ~\cite{bdd-seminal}, this rule follows the standard BDD reduction rules ~in~\cite{bdd-seminal}

    \item Every node $x_i(p)$ is replaced by $y_i(p)$ after beliefs aggregation

    \item the aggregated belief $y_i(p)$ is further propagated and contributes to beliefs aggregations.    
\end{enumerate}


\hl{maybe at the end this is a mapping from one graph to another...}

\paragraph{Belief Reduction and Convergence of Beliefs}
Aggregation and propagation rules leads to reduction of the binary tree where \emph{less experts adopt the belief of most expert one(s)}. 

%\hl{i am not sure whether this should be a lemma or a theorem. }
%\begin{Theorem}[Belief Convergence]
According to the rule defined in~\ref{...}. If we have a sequence of $k$ similar beliefs, that is $[\bar{n} -k,\bar{n}]$ so that $y_{\bar{n}-k} = ... = y_{\bar{n}}$, then all beliefs $n \geq \bar{n}$ will converge (i.e., convergence here means also that peer disagreement  will disappear after the propagation), that is 
$$\forall n \geq \bar{n}, y_{n}  = y_{\bar{n}} = $$


%\begin{proof}
We prove that by induction as follows, 
if we assume it is true at step $n$, this means that $y_{n-1}(p)= y_{n-2}(p)=... = y_{n-k}(p)$ and as a consequence $y_{n}(p) = y_{n-1}(p)= y_{n-2}(p)=... = y_{n-k}(p)$

Now let us prove it for step $n+1$, that is we need to prove that  $y_{n+1}(p) = y_{n}(p) = y_{n-1}(p)= y_{n-2}(p)=... = y_{n-k}(p)$.  According to the rule in ~\ref{..}, $ y_{n+1}(p) = x_{n+1}(p) \neq y_{n-1}(p), ...$ when there exist one $i,j$ so that $ y_{n+1}^{i} \neq  y_{n+1}^{j} $, in this case, according to the rule $i$ does not change its own belief and $ x_i(j) = y_{n+1}^{j}$  or $x_i(j) = y_{n+1}^{j}$. Now we know from the previous iteration that beliefs from $y_{\bar{n}-k} = ... = y_{\bar{n}}$ agree (this is our assumption) and we know as well that $y_{n+1}^{i}$ also agrees with the previous $k$ based on rule\ref{...} (either belief was the same as the previous k or just changed). In this case, we know that all beliefs $y_{\bar{n}-k} = ... = y_{\bar{n}}, y_{\bar{n+1} }$ agree which will lead to a convergence of beliefs (CQFD).  
%\end{proof}
%\end{Theorem}

\hl{if course the convergence is rule dependent and one can want to proof that for a different rule, but this convergence criteria is always good to have because this will as well determine the real-time and efficiency metric of this approach.}


\hl{Selma: i stopped here!}

\paragraph{Beliefs Reduction and Resiliency }
Due to the collaboration and the aggregation function, some autonomous systems adopt the beliefs of others autonomous systems which are more experts, thereby discarding their own belief which disappears from the tree of beliefs (or does not participate anymore to the decision tree). In this case, we are resilient to errors except if experts are making an error. It is clear from the aggregation function that we are resilient to experts $s_{n-1}, s_{n-2}, ..., s_{n-k}$ making an error simultaneously. Where an error can be defined when a belief does not match the ground truth, that is, 

$$y_i(p)\text{ xor } T(p)$$




==> tex/intro.tex <==
%\section{Introduction}

Cooperative driving currently leverages Vehicle-to-X (i.e., vehicle to vehicle and/or vehicle to
infrastructure) communication technologies aiming to carry out cooperative functionalities, such
as cooperative sensing and cooperative maneuvering\footnote{The first fully automated driving car performing automated valley parking and completely relying on infrastructure has been recently released: https://www.bosch.com/stories/autonomous-parking-in-parking-garages/}. Today, infrastructure to support Device-Edge-Cloud Continuum enables sharing of information between distributed (autonomous)
systems and infrastructure~\cite{MundhenkHHZ22,keynote_Date2023}. Broadcasting information from every vehicle using for instance collective awareness messages is thereby enabled. Every vehicle can later make a decision locally or globally, like maneuvering, based on collected information. The fact, however, that there is an infrastructure to share information does by no means imply that the issue of safety and correct collective behavior is assured.
There is a lack for structured and systematic processes and methods to collectively reason about the shared information in order to improve safety, trustworthiness and good
decision making using collaboration in autonomous systems. \hl{emphasize the utility aspect of this: emphasize in particular the need for computable structures to do that.}


 \begin{itemize}
        \item \hl{Introduction: (around 100 readers)}
        \begin{itemize}
            \item \hl{1 page}
            \item \hl{ the introduction is to tell the reader} \textbf{why they should read your paper}
            \item \hl{DO NOT Give the background!}
            \item \hl{DO NOT give them very general known problems in the intro, focus on THE PROBLEM you would like to solve and convey why this is needed.  (DO NOT DEsctibe Mont Everest!)}

            \item \hl{so content wise, your introduction should ONLY include:}
            \begin{enumerate}
                \item  Describe the problem, give an intuition (not a formal description), give an example if you like this is always good, and why this is an interesting problem (from a UTILITY problem). 
                \item State your Contribution ....\textbf{and thats all}: write what your paper delivers, it is a sort of menu in a restaurant :)
                \begin{itemize}
                    \item \textbf{Your Contribution is somehow your specification you can write them at the beginning!}
                    \item Do NOT let the reader GUESS what Your Contribution is!
                    \item put a bullet point as list of contribution!
                    \item put a claim and provide evidence that can be refutable. Some examples are (BE SPECIFIC!): 
                    \begin{itemize}
                        \item "we give the syntax and semantic of a language that supports concurrent processes (Sec 3). Its innovative features are...."
                        \item we prove that the type system is sound, and that type checkig is decidable (Sec4)
                        \item we have built a GUI toolkit in WizWoz, and used it to implement a text editor (Sec 5). The result is half the length of the java version
                    \end{itemize}
                    \item DO NOT put the paragraph in section1, in sec2 ...etc.  INSTEAD \textbf{use forward references from the narrative in the introduction}, the intro should survey the whole paper and therefore forward reference every important part of it! 
    
                \end{itemize}
            \end{enumerate}
       
    \end{itemize}



\section{Assured Autonomy Using Collective Intelligence}
%\subsection{The Challenge of Safe Autonomous Systems in Open Context}
Autonomous systems have the ability to interact with the environment and act independently by solving complex tasks without human intervention. While designing systems, that are able to do well-defined (repetitive) tasks, like automata, is not new, the main current challenge with designing autonomous systems is to provide them with the ability to operate correctly and safely in dynamic and open contexts. That is performing tasks at operation time in an environment that is uncertain or was not fully known or defined at design time. In such environments, autonomous systems must as well \emph{self-decide}. However, when extended to fields like automated driving, where safety is a major requirement, assuring high levels of trustworthiness and good decision making in complex environment becomes a necessity. There is currently a tremendous need to design approaches to reason about safety at operational time.

Cooperative driving currently leverages Vehicle-to-X (i.e., vehicle to vehicle and/or vehicle to
infrastructure) communication technologies aiming to carry out cooperative functionalities, such
as cooperative sensing and cooperative maneuvering\footnote{The first fully automated driving car performing automated valley parking and completely relying on infrastructure has been recently released: https://www.bosch.com/stories/autonomous-parking-in-parking-garages/}. Today, infrastructure to support Device-Edge-Cloud Continuum enables sharing of information between distributed (autonomous)
systems and infrastructure~\cite{MundhenkHHZ22,keynote_Date2023}. Broadcasting information from every vehicle using for instance collective awareness messages is thereby enabled. Every vehicle can later make a decision locally or globally, like maneuvering, based on collected information. The fact, however, that there is an infrastructure to share information does by no means imply that the issue of safety and correct collective behavior is assured.
There is a lack for structured and systematic processes and methods to collectively reason about the shared information in order to improve safety, trustworthiness and good
decision making using collaboration in autonomous systems. \hl{emphasize the utility aspect of this: emphasize in particular the need for computable structures to do that.}


Collaborative aspects in autonomy exploiting cooperation between autonomous multi-agent
systems and their interaction to solve tasks and maximize utility have been proposed
in several work such as~\cite{multiagent}. Collaborative autonomy can be defined as the principle
underpinning collaborative intelligence through which individual contributors maintain their
roles and priorities as they apply their unique skills and leadership autonomy in a problem-solving process~\cite{Gill11}. 
%
Collaborative autonomy therefore recognizes that autonomous
systems (or agents) have different capacities, of for instance, pattern recognition, and a consensus\footnote{A consensus approach usually assumes that autonomous agents are homogeneous.} in reaching collaborative intelligence (as traditionally applied in autonomous multi-agent systems) becomes not always required.

When referring to autonomous systems, the term trustworthiness can be defined considering different parameters~\cite{trustworthiness_as}. 
We refer so far to collaboratively increased trustworthiness and reliability in the following sense: the reliability of an autonomous system increases as its processes for gathering information becomes more accurate,  i.e., lead to a more correct representation of the environment. 
A failure can be defined as an error in an information about the environment that an autonomous
system makes compared to the rest of the group (e.g., due to a misclassification in the perception system). 


Instead of individually relying on own individual sphere of knowledge, autonomous systems operating in the same environment can share information about the environment (e.g., in the form of statements like: "an object has been detected" or "distance to this object is less than 500 m", that can be formulated as propositions or predicates). % to increase collaboratively trustwrothiness in the perceived environment. 
 By sharing and exchanging information (totally or partially), the level of trustworthiness in the environment model that leads to good decision making can be collaboratively increased as the sphere of collective knowledge also increases, see Fig~\ref{fig:collaborative_trustworthiness}.   
However more knowledge, aggregated or inferred by the group, does not systematically lead to a better knowledge. 
We need automated collective reasoning methods for defining rules to systematically infer knowledge collectively, as well as decide about the suitable\footnote{Suitable here refers to the group of autonomous systems that are more trustworthy than others in providing better information about the environment. A more formal definition of these notions will be presented in the next sections. } group of autonomous systems that helps improve collaboratively reliability and  decision making process. 


\begin{figure}
	\centering
  \includegraphics[scale = 0.45]
{figures/collaborative_trustworthiness3.png}
	\caption{Increase collaboratively reliability exploiting collective knowledge that can be expressed as predicates.}
	\label{fig:collaborative_trustworthiness}
\end{figure}


When considering the analogy with humans, reasoning in groups is what humans do regularly in their daily lives to collect more knowledge and improve their decision making process, considering in addition to own opinion, other opinions (often from heterogeneous groups) of individuals with different expertise and different features%\footnote{ more accurate definition of expertise and features in the context of autonomous systems will later be presented.}
. Social epistemology and in particular belief propagation deals with the study of how "good" knowledge and belief propagates in a society~\cite{sep_epistemology_social}. 
The main idea of this paper is to increase reliability and good decision making for autonomous systems exploiting  collective sharing of information. For that, we exploit the premise that autonomous systems have different quality of features which make them eligible for different levels of expertise when sharing information. 
We borrow concepts from social epistemology and provide a \emph{computable and efficient} structure for belief aggregation and propagation. We define the term \emph{collaborative trustworthiness} where an autonomous system can involve two or more \emph{trustworthy} autonomous systems beliefs (on the environment) to possibly form new correct beliefs. This forming or change of belief is based on rules for good decision making, the goal is to increase collaboratively reliability of decision making of each autonomous system. Computability becomes an issue since good decision making needs to be done in real-time. In our case, we rely on lattice to keep track of ranking based on autonomous systems features and to identify which autonomous systems are more trustworthy. We as well consider Binary Decision Diagrams (BDDs) as efficient computation structures for belief aggregation and propagation. 
%\hl{todo: we should emphasize that computability is an issue for  this good decision making needs to be done in real0time, that is why we need \emph{efficient} structures for computations, in our case, we rely on the lattice to keep track of the ranking and we as well consider BDDs as efficient structures for computations (reference the arxiv paper) }
%\hl{emphasize why is this an interesting problem from a utility perspective..}
The contribution of the paper can be structured as follows,
%\hl{ write what your paper delivers as a list of claims for which you will provide evidences (like proofs, experiments, usecase etc)}
\begin{itemize}
     \item Considering concept of social epistemology, we define and formalize the structure of autonomous systems, a notion of expertise and ranking based on the feature to define which autonomous system is trustworthy and contributes to belief aggregation and propagation, considering binary decision trees, the overall idea is sketched in Sec.~\ref{sec:overall_idea}. 
         
    \item we formalize and define a model of computation for belief aggregation and propagation based on well-defined rules in Sec.~\ref{sec:moc_model}. The notion of collaborative trust and related reliability are as well defined. We later present the notion of BDD transformation and reduction resulting from the resolution of peer disagreement. 

    \item Experimental evaluation and validation is presented in Sec.~\ref{sec:exp}. We implement that testing different rules and test how the level of reliability increases considering the collaboration. We investigate in particular how the quality of the group influences the overall results, that is the choice of the group of interest which will contribute to good decision making. Results show that reliability can be improved by a maximum factor of \hl{XX} considering the collaboration and compared to relying on own information.  

   \item we discuss in Sec.~\ref{sec:rw} related work and discuss how our approach extends the state of the art as well the benefits and limitations of our approach.
\end{itemize}





%we build a formal machine based on BDDs and graphs for belief propagation from social epistemology
%List of Contributions:
%\begin{enumerate}
%    \item (we define a computable representation of "society" of AS) we provide a \textbf{general} formal model of computation of collaborative trustworthiness and corresponding collaborative reliability using features representation and beliefs propagation using BDDs (in Sec ) and define rules for belief propagation and peer disagreement that have as an objective to collaboratively increase the overall reliability of the collaborative system.
    
%    \item We define the main idea in Sec... through an example of a smart intersection where automated vehicles need to reason about the presence or not of an obstacle. 
%    \item (we define rules for good decision making as to individual change of belief)
    
%    Definition of rules and their application in the propagation of beliefs is presented in Sec.... we consider several rules based on the meaningful subset of opinions or beliefs to consider. The goal is to minimize this set while increasing the level of reliability. We show that rule XY is better than XX in some situations, etc. as relying on other (experts) opinions can be misleading.
%\begin{itemize}
%    \item define the right opinions that count!
%    \item rule: do we change our belief or not.
%\end{itemize}
    
%    \item we implement the proposed approach in a smart intersection example. The results show an overall increased reliability by XY... considering our proposed approach compared to relying on own information. 

%    \item we discuss in Sec .. related work and discuss how our approach extends the state of the art as well the benefits and limitations of our approach. 
    
%\end{enumerate}



 We rely on BDDs (binary decision diagrams) which are the most frequently used representation types or data structure for boolean functions\footnote{seminal paper for using BDDs are from Lee: Representation of switching circuits by binary-decision programs C.Y. Lee Bell Systems Technical J., 38 (1959), pp. 985-999}. 

 We use BDDs as data structures for boolean functions which allows efficient computability. 



==> tex/old_overall_idea.tex <==
Social epistemology and in particular belief propagation deals with the study of how "good" knowledge and belief propagates in a society~\cite{sep_epistemology_social}. This is based on a structuring of the group that can be viewed as a graph, see Fig.,~ \ref{fig: belief-propagation}, where nodes depict individuals in the group and edges are relationships between them. Beliefs can then propagate from one individual to the rest of the group following a set of rules, which determine information and individuals to rely on for reasoning and how beliefs should be weighted. However, one of the main issues in the epistemic sense is to deal with \emph{peer disagreement}. That is, should an individual (or a system) adjust their own belief based on additional knowledge, which can also be contradictory, provided by other peers? In the following, we discuss how similar principles can be applied to autonomous systems.
\hl{todo: emphasize the problem of peer disagreement}

\begin{figure}
	\centering
  \includegraphics[scale = 0.55]
{figures/belief-propagation}
	\caption{Schematic description based on \cite{sep_epistemology_social} of belief propagation in social epistemology using graphs considering individuals and their relationships.}
	\label{fig: belief-propagation}
\end{figure}

\subsection{Structuring the Group or "Society" of Autonomous Systems}
By applying the principles of belief propagation in social epistemology, we first need a way to structure the group (or society) of autonomous systems or agents\footnote{In this paper, we use similarly the terms autonomous systems or agent. }. Since autonomous agents are different w.r.t. the quality of their features, we use this criteria as a mean to define relationships between autonomous agents considering \emph{dominance} of the quality of features. Let us consider a simple example of a smart intersection as depicted in Fig.,~\ref{fig:intersection_features} with four vehicles and considering two features: distance and perception angle. It becomes clear from the example that vehicle $s_1$ (resp., $s_4$) has better (resp. worse) distance to the pedestrian and a better (resp. worse) perception angle compared to other vehicles. Both $s_2$ and $s_3$ are not comparable since $s_2$ has a better perception angle but a larger distance to the pedestrian compared to $s_3$, while for $s_3$ it is the opposite. We can therefore provide a ranking of all vehicles present in the intersection based on the quality of their features.  We formulate that structure using a \emph{lattice} as a formal representation for partial ordering, with an infimum and a supremum that constitute autonomous agent with worst and best quality of features respectively, see Fig~\ref{fig:lattice}. 


\begin{figure}
	\centering
  \includegraphics[scale = 0.65]{figures/lattice-example1.png} 
% \includegraphics[scale = 0.4]
%{figures/lattice-example}
% \includegraphics[scale = 0.4] {figures/lattice-example1}   lattice-example1 is the figure without the lattice with 4 agents.
	\caption{ Example of autonomous systems operating in the same environment a) vehicles with different features (distance and perception angle) possibly detecting a pedestrian, b) ranking between vehicles based on their features (assuming that the smaller is the value of the feature and the better the quality is).}
	\label{fig:intersection_features}
\end{figure}

\begin{figure}
	\centering
  \includegraphics[scale = 0.55]
{figures/expert-lattice}
	\caption{Lattice as a formal representation of partial-order relationship between autonomous systems based on their features. Green (resp. red) area represent autonomous systems with better (resp. worse) quality of features than $s_4$.} % $\{s_4, s_5, s_6\}$ are incomparable as each  }
	\label{fig:lattice}
\end{figure}

\subsection{Notion of "Expert" in Autonomous Systems}
Considering ranking of autonomous agents based on the quality of their features, a notion of "expertise" can be defined to qualify autonomous agents of a better quality. For every autonomous system with a given quality of features (e.g., $\{s_4\}$ in Fig,~\ref{fig:lattice}), experts are the set of points whose quality dominate its quality for every feature (e.g., $\{s_1, s_2, s_3\}$). Other autonomous agents whose quality of features are dominated by this point can be referred to as less experts. In fact, every autonomous system may still provide a given useful information/knowledge and may have some level of expertise.

\subsection{Structuring the Beliefs as Binary Decision Trees}

We models beliefs as boolean variables. Therefore, for every autonomous system, a boolean variable represent a belief on a given proposition, e.g., “an object has been detected”. We further use Binary Decision Diagrams (BDDs) to model all possible beliefs from all autonomous systems referring to a given proposition. Fig~\ref{fig:bdd_example} depicts an example with 3 autonomous systems. Every vertex is a boolean variable representing the belief of one autonomous system, every vertex has two arcs, either the belief is assigned 1 (true) or assigned 0 (false). Each terminal vertex is labelled 0 or 1 which corresponds to the belief of the \emph{last} autonomous system. 

\begin{figure}
	\centering
  \includegraphics[scale = 0.45]
{figures/BDDs_example}
	\caption{Binary Decision Diagram (BDD) considering 3 autonomous systems.  Decision variables for autonomous system are ranked from the most expert to the least expert one. }
	\label{fig:bdd_example}
\end{figure}

\subsubsection{Beliefs Aggregation and Propagation}

Every autonomous system receives beliefs from other autonomous systems belonging to a group of interest that can be defined based on different rules or procedures. When for example the majority rule is used, the group of interest correspond to all autonomous systems.  When an expert-based rule is used, then the group of interest refers to a (sub)set of experts. A more detailed definition will be presented in Sec.~\ref{sec:moc_model}. Every autonomous system can change its own belief after applying an aggregate function. The goal of the aggregate function is to reduce peer disagreements where an autonomous system can change its own belief to adopt the belief of the rest of the group of interest, i.e., for instance the opinion of more experts nodes. Fig~\ref{fig:aggregate_function} depicts an example of such aggregate function under peer disagreement. In this case the autonomous system $i$ changes its belief when this latter disagrees with all beliefs from other autonomous systems belonging to the group of interest. 

By reducing peer disagreement and adopting the beliefs of other autonomous systems when they contradict with own belief, we aim at reducing errors (e.g., from one autonomous system perception system) by relying on beliefs from other members of the group. The goal is to therefore increase reliability collaboratively. Note that by adopting the belief of other members of the group, an autonomous system is generally resilient to errors except for the case when multiple members of the group of interest are making errors simultaneously. A more detailed discussion regarding the choice of the group of interest, the aggregation rule and reliability will be presented in Sec.~\ref{sec:moc_model}.



\begin{figure}
	\centering
  \includegraphics[scale = 0.45]
{figures/aggregation}
	\caption{Example of an aggregate function for belief aggregation. The function considers $k$ input beliefs $y_j(p)$ on a proposition $p$.  Belief of a node $x_i(p)$ is changed if there is a disagreement with all input beliefs.}
	\label{fig:aggregate_function}
\end{figure}

\subsubsection{Reduction of Beliefs}

The adopted order of variables in the BDDs structure follows a total order from the lattice. In this case, belief propagation in the BDDs starts from the most expert to the least expert node (or autonomous system). The aggregation function is then used by every node in the BDD to decide whether the autonomous system changes its own belief to adopt the belief of the most expert one(s). The aggregated belief is further propagated and contributes to later beliefs aggregation. 

Belief aggregation and propagation lead to a transformation of the BDD to a simpler form as depicted in Fig.~\ref{fig: ....}, where less experts adopt the belief of the most expert one (s). In that case terminal vertices correspond to the belief of the last autonomous system(s). which allows to reduce as well the complexity of systems. 


\hl{at the end of this section say that the following sections will present a detailed model and formalization of this and that the experimental section will evaluate x and y.}

\begin{figure}
	\centering
  \includegraphics[scale = 0.45]
{figures/BDDs_Reduction}
	\caption{(a): non reduced BDDs, (b): reduced BDD considering the most expert rule, (c) reduced BDD considering the 2-experts rule.}
	\label{fig: ...}
\end{figure}







==> tex/overall_idea.tex <==
%\section{Explain the overall idea}
\section{Exploiting Collaborative Trustworthiness for Safe Autonomous Systems (4 pages)}
\label{sec:overall_idea}

\begin{itemize}
        \item \hl{Present Your Idea! (2 pages): Explain your Idea, the readers are very eager to read your idea!}
        \begin{itemize}
            \item \textbf{Explain it as if you want to explain it on the BOARD and VERBALLY!}
            \item First: give an intuitive explanation of your Idea (BEfore the DEfinition!)
            \item USE EXAMPLES! as if you would as well do it on the board
            \item At the definitions as well!
            \end{itemize}
\end{itemize}


\subsection{Simple Example for Our Proposed Collaborative Trustworthiness}

%\begin{figure}
%	\centering
%  \includegraphics[scale = 0.3]
%{figures/simple_example}
%	\caption{Simple example of 3 autonomous systems operating in the same environment and having different distances and perception angles to a given pedestrian.}
%	\label{fig:simple_example}
%\end{figure}

\begin{figure}[!htb]
\minipage{0.32\textwidth}
  \includegraphics[width=\linewidth]{figures/simple_example}
  \caption{Simple example of 3 autonomous systems operating in the same environment and having different distances and perception angles to a given pedestrian.}\label{fig:awesome_image1}
\endminipage\hfill
\minipage{0.32\textwidth}
  \includegraphics[width=\linewidth]{figures/quality_features_simple.png}
  \caption{A really Awesome Image \hl{maybe start as Dirk suggested with the results to motivate the rest}}\label{fig:awesome_image2}
\endminipage\hfill
\minipage{0.32\textwidth}%
  \includegraphics[width=\linewidth]{figures/bdd_simple.png}
  \caption{\hl{maybe put rather an example like slide 20}}\label{fig:awesome_image3}
\endminipage
\end{figure}

\begin{figure}
	\centering
  \includegraphics[scale = 0.65]{figures/lattice-example1.png} 
% \includegraphics[scale = 0.4]
%{figures/lattice-example}
% \includegraphics[scale = 0.4] {figures/lattice-example1}   lattice-example1 is the figure without the lattice with 4 agents.
	\caption{ Example of autonomous systems operating in the same environment a) vehicles with different features (distance and perception angle) possibly detecting a pedestrian, b) ranking between vehicles based on their features (assuming that the smaller is the value of the feature and the better the quality is).}
	\label{fig:intersection_features}
\end{figure}




%Let us consider the following simple example depicted in Fig~\ref{fig:simple_example}. The example is used for illustration purposes of the main idea of the paper and will be used to give an intuitive explanation of the addressed problem and proposed solution. 
%


%The example considers 3 autonomous systems operating in the same environment, which contains as well a pedestrian.

\hl{let us consider that all autonomous systems receive the same information and that no autonomous systems sends two different information to two different other autonomous systems. --> maybe at the end is to consider no malicious attack or so}

\hl{defining consistency conditions is something different: in leslie lamport case, conditions are : 1) all experts should say the same thing, 2) a small number of traitors (low expert guys in our case) cannot cause the loyal generals to adopt a bad plan ... there are things he called \textbf{interactive consistency conditions}}




Let us consider the following simple example of 4 autonomous systems like vehicles operating in the same environment like a smart intersection, which contains as well a pedestrian as depicted in Fig.,~\ref{fig:intersection_features}.
Note that autonomous systems having different features in terms of different distances and different perception angles w.r.t a pedestrian that needs to be detected. The aim of each autonomous systems is to safely progress towards their goals without colliding with the pedestrian. For that an early detection of the pedestrian is required. We therefore consider so far simple statements which can be viewed as well as predicates such as "a pedestrian has been detected".  Depending on individual perception system, an autonomous system can output either true or false to such statements.  

%a smart intersection as depicted in Fig.,~\ref{fig:intersection_features} with four autonomous vehicles.  and considering two features: distance and perception angle. 


%The example considers 3 autonomous systems operating in the same environment, which contains as well a pedestrian. 

%Note that autonomous systems having different distances and different perception angles w.r.t a pedestrian that needs to be detected. The aim of each autonomous systems is to safely progress towards their goals without colliding with the pedestrian. For that an early detection of the pedestrian is required. We therefore consider so far simple statements which can be viewed as well as predicates such as "a pedestrian has been detected".  Depending on individual perception system, an autonomous system can output either true or false to such statements.  

We would like to infer a good decision process based on information collaboratively shared between autonomous systems. In particular for cases where some autonomous systems conclude that they have seen a pedestrian and not the other ones. When information has been shared, once can directly conclude, for instance based on a voting principle or majority rule, that a pedestrian has been seen in case 2 autonomous systems have actually detected it and not the third one. This "judgement"\footnote{Since we use concepts from social epistemology, we also borrow some terminology from this domain that we will formally define later. } inferred collectively can be then be used by the third autonomous system to correct its own "belief" and change it from "False" to "true" statement for "a pedestrian has been detected". Based on that, each autonomous system can consider this information to compute a trajectory for safely progress in the environment. The goal is to increase collaboratively the trustworthiness in the environment of operation by increasing reliability and reducing the number of errors performed by each autonomous system, an error being for instance caused by a misclassification of the perception system. 

We refer to the rule, like the above-mentioned majority rule, used to collectively infer a "judgement" as an \emph{aggregate} function. We will show later that the majority rule or the standardly adopted consensus approach in multi-agent systems will not necessarily always lead to a good decision making that is increasing reliability, and if at any time then this comes at the cost of a large communication overhead. We present in the following an alternative solution. The approach is mainly based on the premise that autonomous systems are different.  They have different features like illustrated in the example considering different distances to the pedestrian as well as different perception angles. They therefore can contribute differently to the collective reasoning to reach a good\footnote{Good decision is here used in the sense of correct and "fast" decision.} decision. We therefore exploit different quality of features to establish a ranking among autonomous systems. The ranking is later used to define autonomous systems that are more \emph{trustworthy} than others because they have better quality of features. We will show in the following that this approach offers numerous advantages, and can lead to increased reliability and efficiency. Actually, basing the approach on ranking of autonomous systems allows to first collect the "beliefs" of most trustworthy ones. Therefore, instead of relying on the majority considering the entire group, we can directly rely on a sub-group of most trustworthy autonomous systems, that we refer to as \emph{experts}, to provide an aggregate "judgement". This "judgement" can later further propagate to the rest of the group to be adopted. 

In the above-mentioned example, experts can be autonomous systems closer to the pedestrian (i.e., shorter distance) and having a better perception angle (e.g., trajectory aligned with pedestrian compared to autonomous systems making a turn.). Consider that $s_1$ and $s_2$ have the best quality of features according to the described criteria. %Instead of relying on the majority, 
An aggregate function can be defined relying solely for instance on 2 experts and the aggregated "belief" will then propagate further to the rest of autonomous systems. Note that since we consider a simple example with 3 autonomous systems then not much of a difference can be observed w.r.t a majority rule. If we however extend the number of autonomous systems to 10 or even 100 or more in the same environment, then relying on fewer number of experts rule will show significant benefit in terms of efficiency, and as we will demonstrate reliability\footnote{Relying on experts, that is autonomous systems with better quality of features is mostly enough to lead to a correct statement. However, we will show as well that such rules are not robust to the case where experts make an error of "judgement" which we assume is less likely to happen simultaneously in the reality. A detailed discussion about how reliability is affected by aggregation rules and the quality of considered group of autonomous systems will be presented in the following section. } w.r.t the majority rule.  

\hl{---}
It becomes clear from the example that vehicle $s_1$ (resp., $s_4$) has better (resp. worse) distance to the pedestrian and a better (resp. worse) perception angle compared to other vehicles. Both $s_2$ and $s_3$ are not comparable since $s_2$ has a better perception angle but a larger distance to the pedestrian compared to $s_3$, while for $s_3$ it is the opposite. We can therefore provide a ranking of all vehicles present in the intersection based on the quality of their features. 
\hl{---}

In order to automate good decision making using collective intelligence in terms of collaborative rules for "belief" aggregation and propagation, we need efficient structure of computation. This is in particular very relevant as considered features can change over time and thereby corresponding ranking. Also "belief" propagation requires significant time if the number of autonomous systems is high. We rely in the following mainly on Binary Decision Diagrams (BDDs) as decision trees for automated reasoning. Considering the example of 3 autonomous systems, an example of such tree is depicted in Fig.~\ref{fig:bdd_reduction}, where every node corresponds to a decision variable for an autonomous system, which has two possible "belief" assignment for every statement as "true" (logic 1) or "false" (logic 0).  Starting from a given ranking, we use in particular Ordered Binary Decision Diagrams starting by propagating the "beliefs" from most trustworthy autonomous system to the least trustworthy ones. In order to increase the efficiency of "beliefs" aggregation and propagation, we define in the following reduction rules in order tor educe the size of the binary decision diagram. \hl{Selma: i will see later, maybe add more intuitive explanation with that regard.}

In the following, we generalize and formalize the simple example that we considered so far.

%\begin{figure}
%	\centering
%  \includegraphics[scale = 0.45]
%{figures/BDDs_example}
%	\caption{Binary Decision Diagram (BDD) considering 3 autonomous systems.  Decision variables for autonomous system are ranked from the most expert to the least expert one. }
%	\label{fig:bdd_example}
%\end{figure}






==> tex/related_work.tex <==
\section{Related Work and Research Gaps}
\label{sec:rw}

%\hl{2-4 pages}

% --------------------------------------------------------------
% Christoph: Start with Byzantine Generals Problem as foundation
% --------------------------------------------------------------

Research~\cite{lamport2019byzantine} is a pioneering work in the field of distributed computing and is a classic in the field. It provides a foundational work on distributed systems and consensus algorithms. This paper tackles the complex challenge of achieving consensus in a network of nodes when some of those nodes may be unreliable, malicious, or experiencing Byzantine failures. The analogy of generals coordinating their actions in the presence of traitorous generals provides an intuitive framework for understanding the problem and is a very similar problem to what we are trying to solve.
The problem at hand involves a fault-tolerant algorithm for detecting malicious or malfunctioning agents within a group. Specifically, it is required that more than two-thirds of the generals in the system remain loyal, which typically translates to a setup involving 3m+1 generals, allowing for a maximum of m traitors. An example of a scenario where this problem arises is with the Byzantine army generals. Notably, these generals can only communicate using oral messages. However, it's worth mentioning that with unforgeable written messages, the problem becomes solvable for any number of generals and potential traitors. One key aspect to consider is that solving this problem can be expensive in terms of both time and the number of messages required. It prompts the question of whether more recent research has found more efficient solutions, especially in terms of minimizing message exchanges. When assessing this against our research, we find that our approach is characterized by its requirement of relatively few messages and is not as computationally expensive.

% --------------------------------------------------------------
% Christoph: Continue that some works solve this problem by determining and assigning a notion of trust and trustworthiness to agents within a system. This paper is an overview of all the trust related topics and considerations. We will fork from this into different subsections of trust-research
% --------------------------------------------------------------

\hl{@Christoph: rephrase - taken from collective reasoning paper}
When referring to autonomous systems, the term trustwor-
thiness can be defined considering different parameters~\cite{devitt2018trustworthiness}.


% --------------------------------------------------------------
% Christoph: More works are needed here which determine trust values.
% --------------------------------------------------------------

In the context of the IoT era, machine-machine trust plays a pivotal role. In~\cite{Liu2016MachineTM} a novel machine-machine trust algorithm is introduced, centered around both the transaction/interaction behavior and a computable feedback-rating in the presence of intentional or non-intentional misbehavior. 

The Eigentrust algorithm is a classic in reputation management in peer-to-peer networks~\cite{10.1145/775152.775242}, in order to reduce the number of inauthentic files and to isolate malicious peers. It is based around a unique global trust value that is assigned to each peer, based on their reputation in the network. Due to the computation exploiting the eigenvector of a matrix with normalized local trust values, the entire system's history is taken into account.

An overview over AI based trust models is presented in~\cite{cotronei2023improving}.

% --------------------------------------------------------------
% Christoph: How to determine whether a trust value is "correct"? Refer to the concept of calibrated trust.
% --------------------------------------------------------------

A closely related topic is calibrated trust. Calibrated trust is the measure of how appropriate it is for the operator to trust a given system.  Usually, this concept is considered in human-machine interactions, where the overconfidence of an operator in a system might lead to situations that the system cannot handle. An example is the need for drivers of autonomous vehicles with autonomy level 4, where the driver needs to take over controls within a sufficient time frame. If, however, a driver is not able to take over, because they are asleep for example, there exists an overconfidence in the system. 
On the contrary, underconfidence in a system may lead to a system not being used, which could also lead to information not being received with potential negative consequences. One example of underconfidence in a system is the plane crash on July 2, 1994, of USAir Flight~1016, that was affected by wind shear during landing, which lead to the accident. Preceding the incident, the air traffic controller received three warnings by a wind shear alert system, but due to a lack of trust in the system, send only one warning to the plane, which was never received, killing 37 people.~\cite{kok2020trust}
Calibrated trust means that we need to find the right balance between over- and underconfidence to get optimal results.~\cite{mcdermott2019practical}~\cite{10.1145/2667317.2667330}

In~\cite{mcdermott2019practical}, calibrated trust is determined by comparing the trust of a human in the system with the trustworthiness of the system in certain situations. As most automation does not have a constant performance, situations where the system excels or underperforms are used as calibration points. 
As long as trust and trustworthiness are aligned in those instances, the system is considered trust-calibrated, otherwise, it is adjusted accordingly.

% --------------------------------------------------------------
% Christoph: There is also the possibility to not trust the shared trust value. The concept of "Zero-Trust" means, that every agent needs to "prove" itself to become trustwothy, regardless of its status.
% --------------------------------------------------------------

\hl{@Christoph: In this part it becomes interesting because we talk about the notion of trust and how this is handled possibly in autonomous systems, but here also we should structure that better and position our work better}

In~\cite{buck2021never}, a review of zero-trust is presented, which represents a philosophy in networking security solutions to never trust any participant in a system, even if one is considered an "insider" of the system. Therefore every system needs to be checked to obtain more privileges, which can also be translated into an increase in a systems' trustworthiness.

% --------------------------------------------------------------
% Christoph: What can we do when we do have a trust value that is "correct"? Transition text.
% --------------------------------------------------------------

In communication networks, dealing with a malicious or faulty agent can often be dealt with by ignoring the communication from it. However, in cyber-physical systems, this can potentially lead to even more problems, as the agent is still able to inflict damage, such as enforcing collisions. Therefore, a solution in an AIM needs to be able to react dynamically to malicious behavior. One approach is to assign each vehicle a notion of trust. Trust is a concept studied in a variety of scientific disciplines, such as psychology or philosophy, which is sought to be implemented in machine-machine collaboration. 

% --------------------------------------------------------------
% Christoph: The following work uses a reputation based trust model. Each agent is assigned a value and if an agent with a low reputation is nearby, an agent activated additional safety features, or stops sharing detailed information.
% --------------------------------------------------------------

In~\cite{halasz2022rethinking} a framework is proposed which uses a trust model to determine a trust value for each vehicle, by considering each vehicle's own sensor data and the propagated reputation of other vehicles. 
The trust value is then fed into a safety module which selects an appropriate action from a decision tree. A system with high trust then gets exposed to more data and is also sharing more data of its own. However, when dealing with a malicious vehicle, communication is scaled back according to the rules set in the decision tree. The decision tree itself can either be updated as an update, or by using a self-adaption algorithm.

% --------------------------------------------------------------
% Christoph: Having trust values and decision-algorithms is all good and fine, but it needs to be computed in real-time.
% --------------------------------------------------------------

\hl{@Christoph: reduce - this was taken from the ERC proposal}

Given quickly increasing connectivity and available computation capabilities (e.g., using advanced 5G/6G wireless communication technology and Edge-Cloud-Infrastructures), more future autonomous systems will depend on cooperation in combination with infrastructure. The infrastructure-vehicle cooperative autonomous driving approach relies on cooperation between intelligent roads and intelligent vehicles, which is not only safer but also more economical compared to the traditional on-vehicle-only autonomous driving~\cite{liu2022ieee}. In this case, sharing of information needs to be performed in real-time and guaranteed across compute and communication resources. Hardware and software platforms should therefore, as advocated by CCR, as well support trustworthy and real-time data transmission and processing. It is not sufficient to provide mathematical models of computation for collective reasoning without guaranteeing that assumptions and considered properties are enforced at the platform level. In the past years, a lot of work has been done in the real-time community to guarantee the timeliness of data in safety-critical systems, when sharing compute and communication resources. Providing end-to-end latency guarantees at design time  across computation and communication resources requires in general complex analysis approaches,  such as compositional performance analysis~\cite{hofmann2017cpa},~\cite{easwaran2008compositional}, for bounding the worst-case end-to-end timing behavior. Special attention is often given to cause-effect chains in embedded control systems~\cite{durr2019end}. Authors in~\cite{jacob2016end} propose a distributed protocol that considers the complete transmission chain across multiple resources. Guarantees for end-to-end deadlines are achieved, considering unpredictable changes at run-time, using a set of contracts on elements of the transmission chain based on a worst-case delay and buffer analysis. This approach follows the Logical Execution Time (LET) paradigm where communication and data synchronization follow predefined time schedules, dimensioned taking into account the worst-case execution time of each individual task. We focused in our previous work on innovative aspect in using hardware/software (HW/SW) co-design approaches for controlling the effect of data interference when shared on same platforms, combined with formal methods for the analysis of the performance behavior of complex hardware systems like DRAM memory systems, or networks-on-chips~\cite{saidi2018exploiting}. This combination was extended in~\cite{hamann2020building} to support on-the-fly deployment of safety-critical functionalities on distributed Edge-Cloud-Infrastructure through a framework with a comprehensive system-level abstraction to provide end-to-end quality-of-service (QoS) guarantees. The framework builds on different cross-discipline concepts from cloud computing, networking and embedded real-time domains. To deal with providing guarantees on critical transmissions for highly dynamic resources such as wireless communication, we further provided in~\cite{nota2022providing} the first formulation for the analysis of network slicing, used to isolate applications in 5G/6G with the support of mixed criticality. In~\cite{nota2022context}, I advocated and presented the first formulation for context based worst-case guarantees for wireless communication, where guarantees based on the context of operation are provided. Both real-time and trustworthiness have been identified as Key Performance Indicators (KPIs) in the development of 6G since many applications will rely on supporting communication for (mixed) critical application in the future~\cite{mahmood2021machine}. The fact that there is an infrastructure to share information does, however, not assure the safety issue and correct collective (intelligent) behavior. In addition to real-time requirements, the focus of CCR deals with the semantic of data exchanged used for reasoning and how data can be aggregated to infer good decision making process.

% --------------------------------------------------------------
% Christoph: So far we assumed that the communication is always correct. Continue with works that do not assume correct communication, e.g., in fault-tolerant systems.
% --------------------------------------------------------------

Fault-tolerant control systems (FTCS) refer to systems capable of functioning even when their parameters deviate from an acceptable range, provided that essential conditions are satisfied. Two main categories of FTCS exist: active fault-tolerant control systems (AFTCS), where faults are actively identified and addressed, and passive fault-tolerant control systems (PFTCS), where the system is inherently designed to handle faulty inputs. The efficacy of AFTCS relies heavily on fault detection capabilities and adaptability, making them susceptible to nonlinear systems with uncertainties. In contrast, PFTCS, while less adept at handling a high number of faults, exhibit quicker responses due to their less complex computational architecture. Hybrid solutions combining elements of both AFTCS and PFTCS are not only possible but also commonly employed within systems.~\cite{amin2019review}












% Fault tolerant control systems (FTCS), are defined as systems which are able to operate, even if its parameters are outside an acceptable scope, as long as the necessary conditions are met. FTCS are categorized into active (AFTCS) - meaning faults are detected and actively dealt with - and passive (PFTCS) - meaning the system is build in such a way, that it can inherently handle faulty inputs. The quality of AFTCS depends largely on the systems' ability to detect faults and the adaptability to them, making it vulnerable for nonlinear systems with uncertainties. PFTCS are less capable in terms of the number of faults it can handle, however, due to its less sophisticated computational architecture, it can act faster. 
% Of course, hybrid solutions within a system are also possible and are also common.~\cite{amin2019review}

% \vspace{15pt}

% % --------------------------------------------------------------
% \hl{Christoph: Where to put the digital twin paper from dirk and dirk Elias?}
% % --------------------------------------------------------------


% % Safety in V2I and V2V and AIM
% % Relevant for introduction section as well?
% Over the past decades, several works have been done to increase the safety and efficiency of autonomous and semi-autonomous vehicles with the help of vehicle-to-infrastructure (V2I) and vehicle-to-vehicle (V2V) communication. Due to an increased accident risk at intersections, with more than 40\% of all accidents in the US and Europe taking place at intersections, there is a need for an intelligent intersection management system, also known as autonomous intersection management (AIM)~\cite{8756239}~\cite{azimi2014stip}.

% % Uncontrolled Intersection, rule based approach do clarify order of passing vehciles and according maneuvers such as decelarating
% Many solutions for an AIM establish rules, which dictate the flow of traffic. In~\cite{lu2014rule} a set of priority rules is introduced to resolve conflict situations in an uncontrolled intersection (i.e., without traffic lights) using V2V communication, coupled with a collision avoidance algorithm. This paper offers intuitive laws that humans intuitively follow and formalizes them for the use in semi-autonomous applications. In this paper, however, it is assumed that the information shared in the V2V communication is always correct.

% In~\cite{de2013autonomous} a collision avoidance algorithm is also introduced, which solves sequential local optimization problems by taking the degree of freedom of each vehicle into account. In this work, the concept that different vehicles have different characteristics is taken into account. Here, it is also assumed that the cars communicate only their reaction time and a timestamp when a car enters the intersection and that the communication is also always correct.

% % Virtual Intersection V2V Communication
% In~\cite{9707738}, a cooperative dynamic intersection protocol is presented. A dynamic intersection definition, which means there is a potential collision point that is not available in a database, is also presented. As this research follows a dynamic protocol, a centralized approach is unfeasible, as such intersections can appear anytime, anywhere. Therefore, a V2V approach is used, in which connected autonomous vehicles use the assigned priority to each lane to determine who goes first. Stopping is not needed, due to the on-board perception systems. The study, however, assumes that the perception works perfectly every time. 

% % Resilience Monitoring Framework
% In~\cite{9653143} a resilience monitoring framework for a heterogeneous team of robots is described. It allows for the reconfiguration of shared resources that are used in the team after individual components have failed. The work introduces the notion of one-hop observability, which means that the robots can identify that a resource has failed based on the abstracted performance.
% \hl{---> end}
















































 
% continue from this paper here
%As safety is a major concern for an AIM, several research has been done in this area.

% Different degrees of freedom of each agent -> different features
% local optimization problem is solved for each vehicle with different contraints
% reduce accidents 



% Fazlt Tolerant Networks for vehicluar systems

%Spatial Redundancy

% Information Redundancy




%Fault tolerance distributed systems

% multo agent syste,s

% consensus bases syste,s 
% automomous ahgents

% collective reasoning 




% In order to be confident in the abilities of such a system, the intended user needs a certain level of "trust" in the system, regarding several factors, such as safety or efficiency. \cite{mcdermott2019practical} \hl{OTHER SOURCES AS WELL}
% However, not only needs the intended user trust in a system, the system itself needs to have some form of justification for a notion of "trustworthiness". Trustworthiness now is a measure how well an operator trusts a system and how much the operator should trust this system. If operators are aware of the pros and cons of a system, they can judge the systems capability appropriately. \cite{mcdermott2019practical} 
% It is important to note that the trustworthiness of a system is a dynamic value and changes over time. Think of a day with good driving conditions (sunny day, little traffic) and compare it with bad driving conditions (slippery road, fog). The trustworthiness of an autonomous vehicle changes accordingly.

% Calibrated trust is the measure how appropriated it is for the operator to trust the system. 
% Overconfidence in a system is dangerous as it can result in situations that the system can not handle. 
% under confidence in a system may result in information not being used and therefore this can also lead to dangerous situations. under confidence is also bad, for example, when a human has under confidence in a self driving car, he or she may not use it calibrated trust means that we need to find the right balance between over and under confidence to get optimal results




% \hl{position your self with respect to others, give credit to other work as well!, talk about your limitation in comparison to other work}

% \begin{itemize}
%     \item talk about calibrated trust
%     \item approaches from the fault tolerance domain like the paper from Leslie Lamport. 

%     \item https://arxiv.org/abs/2205.10864
%     \item collective reasoning
%     \item https://arxiv.org/abs/2212.01354

% \end{itemize}

%\href{https://dl.acm.org/doi/pdf/10.1145/2459976.2460035?casa_token=M5lKXczhK18AAAAA:Xl4ovBq3xzXS2iYNa-Pup2TRYi1BKdPvnc6_DLvcZpioxZEBNdDY5v7hX8nbib00UDzXJSQ0rHN8}           

% A related topic to this work is 

% Other works also touch on similar topics. One topic is calibrated trust.

% In autonomous systems, automation and AI can be found in many applications nowadays. One prevalent example of such systems are autonomous driving vehicles, which are foreseen to be used extensively in the future. \hl{SOURCE}





% The users of autonomous systems need a certain level of trust in order \cite{mcdermott2019practical} 

% calibrated trust:
% \begin{itemize}
%     \item over confidence in a system is dangerous as it can result in situations that the system can not handle.
%     \item under confidence in a system may result in information not being used and therefore this can also lead to dangerous situations
%     \item under confidence is also bad, for example, when a human has underconfidence in a self driving car, he or she may not use it 
%     \item calibrated trust means that we need to find the right balance between over and under confidence to get optimal results
%     \item source: %\href{https://www.bosch.com/stories/calibrated-trust-in-automated-driving/}
% \end{itemize}

% Fault tolerance domain from Leslie Lamport:
% \begin{itemize}
%     \item Fault tolerant algorithm to detect malicious or malfunctioning agents in a group
%     \item more than two-thirds of the generals need to be loyal e.g. 3m+1 generals, max m traitors
%     \item example: generals of the byzantine army
%     \item communicating only by oral messages
%     \item with unforgeable written messages the problem is solvable for any number of generals and possible traitors
%     \item source: The Byzantine Generals Problem by Leslie Lamport
%     \item expensive in amount of time and messages required
%     \item perhaps newer research where this is better?
%     \item compare with our research: few messages required, not expensive?
% \end{itemize}

% Federated Learning Aggregation: New Robust Algorithms with Guarantees:
% \begin{itemize}
%     \item machine learning models are trained on several clients
%     \item the trained models are then collected and aggregated with an algorithm to get an "average" model
%     \item the "average" model is then distributed to the clients and again trained
%     \item then repeated?
%     \item continue ...
% \end{itemize}

% In \cite{https://doi.org/10.48550/arxiv.2205.10864} multiple machine learning models are trained on several clients and thus the model is exposed to a greater variety of situations. Using an aggregation function, the trained models are collected and combined into a more general "average" model, which is ought to be more robust against ... . This procedure is repeated several times, until a satisfactory result is obtained.




% Designing Ecosystems of Intelligence from First Principles:
% \begin{itemize}
%     \item 
% \end{itemize}

% Assessing Trustworthiness in Collaborative Environments:
% \begin{itemize}
%     \item At the example of Wikipedia article edits, it is investigated whether one user can be trusted based on their edit history
%     \item in collaborative environments without an explicit authority, the quality of information is unknown 
%     \item community based user trust and document trust of Wikipedia articles

%     \item "important to associate trust values with information exchanges across a disparate set of collaborators"
%     \item two coarse-grained categories: 
%     \item consensus-based models: for example award culture on Wikipedia for authors
%     \item Calculating trustworthiness in collaborative set of actors by:
%     \item Transitivity: Trusted users produce trusted content, trusted content is produced by trusted users
%     \item Circularity: two transitivity statements must be able to handle circular relationships like this one: (A -> B -> C -> A). This should stop and not go on forever when investigating trust
%     \item Roots of trust: one way to break these cycles is by finding roots of trust that provide an initial anchor point of trust assignments
%     \item Authoritative models: organizational charts, control policies
% \end{itemize}

% In \cite{10.1145/2459976.2460035} the trustworthiness of users is determined in a collaborative environment. The example is given at simple English Wikipedia articles. There, users award other users awards when they make good work, such as a good revision of an article or writing a good new article. Articles can also receive an award such as " good article " or " very good article" (Check names). If a user contributed to such an article, its ranking gets better (? check again). The algorithm tries to determine whether the next contribution of a user will be reverted or not. The algorithm has a pretty high accuracy (give number). The shortcomings of the algorithm are that if a user is very knowledgeable in one field but not so much in another field, the ranking (?) for both fields is mixed, making the ranking less reliable. In future works there are going to be distinctions between topics. (Too much? this is outlook) 





% In \cite{10.1145/3004323.3004326} introduces a framework where trust calibration is done for sub-tasks of autonomous driving vehicles. 
% \begin{itemize}
%     \item Divides system into functional levels
%     \item operational level: lowest level of driving functions such as braking blinking checking mirrors etc.
%     \item tactical level: "maneuvers" such as overtaking, a combination of multiple operational level functions
%     \item strategic level: e.g. route planning 
%     \item uses trust / distrust in other agents
%     \item does NOT include context such as weather, drivers condition etc
% \end{itemize}

% The drivers need to know what their vehicle is and is not capable of. They then react properly when handover request occur.
% This might indicate different capabilities of different cars -> similar to our new idea?


% Social epistemology:




% % Fault Tolerant Cooperative Control (FTCC) for Multi Agent Systems (MAS)

% \cite{yang2019fault}




% gravity points

==> tex/system_model.tex <==
\section{System Model: Autonomous System, Features and Beliefs}

Social epistemology and in particular belief propagation deals with the study of how "good" knowledge and belief propagates in a society~\cite{sep_epistemology_social}. This is based on a structuring of the group that can be viewed as a graph, see Fig.,~ \ref{fig: belief-propagation}, where nodes depict individuals in the group and edges are relationships between them. %Beliefs can then propagate from one individual to the rest of the group following a set of rules, which determine information and individuals to rely on for reasoning and how beliefs should be weighted. 
We propose an approach to increase reliability of autonomous systems by relying on collective knowledge (i.e., so far "beliefs"\footnote{A more formal definition of the notion of beliefs is presented later.} from other autonomous agents). For that, we first structure using graph models autonomous systems based on the quality of their features. We later propose a model of computation for belief aggregation and propagation using boolean algebra, where every autonomous agent formulates an output belief (which will be further shared and propagated) based on its own belief and other inputs beliefs from other autonomous agents \footnote{An own belief can be the output of an autonomous systems perception system for instance. The formed output belief based on collective knowledge is the one that will be further shared to contribute to forming the beliefs of other systems.}.   In order to form a belief, every autonomous system can maintain its own belief or change it according to inputs peers. The belief is further propagated to other autonomous systems and will contribute to other systems beliefs. We define in the following precise rules for forming and propagating beliefs.  

%\hl{Selma: todo i should structure this section a little bit into definitions and the rest like the RTSS, i do not need to add lemma or theorem in this case, let us consider definitions just for the notions or notations or terms, all the rest is not definition}



\subsection{Autonomous Systems, Features and Beliefs}

\input{tex/definitions}
